A Perspective on the Foundations of Derived Analytic Geometry

We show how one can do algebraic geometry with respect to the category of simplicial objects in an exact category. As a biproduct, we get a theory of derived analytic geometry.

==> chap10applicationsfurtherwork.tex <==

\chapter{Applications and Further Work}\label{AFW}

\section{Some Applications and Further Work}

In this final chapter we present some future applications to mapping stacks and quotient stacks, and discuss some other future work.






%is a biholomorphism. Consider the collection of maps $\{U_{i}\rightarrow X\rightarrow [X\big\slash G]\}$. 
%For each $x\in X$ choose a neighbourhood $U_{x}$ of $x$ such that $U$ is invariant under $\mathrm{Stab}_{G}(x)$, $U_{x}\cap(\gamma.U_{x})=\emptyset$ for $\gamma\notin\mathrm{Stab}_{G}(x)$, and 
%
% Let $U_{i}\rightarrow X$ be a cover of $X$ such that $G(U_{i})\cap U_{i}=

  

%   It acts transitively on $\mathbb{A}_{an}^{1}\setminus\{0\}\defeq\mathrm{Spec}(\mathcal{O}(w,w^{-1}))$ by $(z,w)\mapsto e^{2\pi iz}w$. The stabiliser of $1$ is $\underline{\mathbb{Z}}$. Moreover $\underline{\mathbb{Z}}$ acts freely on $\mathbb{A}^{1}$. 
%   Thus we have
%   $$\Bigr[\mathbb{A}^{1}_{an}\big\slash\underline{\mathbb{Z}}\Bigr]\cong\mathbb{A}^{1}_{an}\setminus\{0\}$$
% Hence the exponential map $\mathrm{exp}:\mathbb{A}^{1}_{an}
% Now the map $\underline{\mathbb{Z}}\rightarrow\mathrm{Spec}(\mathbb{C})$ is a covering map. In particular it is flat \'{e}tale.
% 
%  Thus by Remark \ref{rem:quotprops}, the exponential map
% $$\mathrm{exp}:\mathbb{A}_{an}^{1}\rightarrow\mathbb{A}_{an}^{1}\setminus\{0\}$$
% is flat \'{e}tale.

  

==> chap7generalisedgeom.tex <==

\chapter{Generalised Derived Algebraic Geometry}\label{GDAG}

\section{A General Formalism for Derived Algebraic Geometry}

In this section we give a general axiomatic schema which incorporates both the structured spaces and relative monoidal approaches to geometry, and permits many common constructions. In particular there is a good formalism of cotangent complexes and obstruction theories.

\begin{defn}
A \textit{pre}-$(\infty,1)$-\textit{algebro-geometric tuple} is a tuple 
$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{Mod},\mathrm{sqz})$$
 where
\begin{enumerate}
\item
$\mathbf{Str}:\mathbf{Aff}\rightarrow\mathbf{Cat}$
is a $\mathbf{Cat}^{\mathbf{R},acc}$-presheaf, such that for any $f:X\rightarrow Y$ in $\mathbf{Aff}$, $f_{*}\defeq\mathbf{Str}(f)$ commutes with finite limits.
\item
$$\mathrm{Spec}:\mathbf{Str}\rightarrow {}_{(-)\big\backslash}\mathbf{Aff}^{op}$$
is a natural transformation of presheaves of categories which is termwise a right adjoint, with left adjoint $\mathrm{Spec}^{*}$
\item
$$\mathcal{O}:{}_{(-)\big\backslash}\mathbf{Aff}^{op}\rightarrow\mathbf{Str}$$
is a natural transformation of presheaves of categories which is termwise a right adjoint, with left adjoint $\mathcal{O}^{*}$.
\item
$\eta$ is a natural equivalence between the identity transformation and the composition
\begin{displaymath}
\xymatrix{
\mathbf{Str}\ar[r]^{\mathrm{Spec}}&{}_{(-)\big\backslash}\mathbf{Aff}^{op}\ar[r]^{\mathcal{O}} & \mathbf{Str}
}
\end{displaymath}
\item
$\mathbf{Mod}:\mathbf{Aff}\rightarrow\mathbf{Cat}^{\mathbf{R},acc,t,c,e}$ is a presheaf of categories.
\item
$\mathrm{sqz}:\mathbf{Mod}\rightarrow\mathbf{Str}$
is a natural transformation.
%\item
%$$\mathbf{QCoh}:\mathbf{Aff}^{op}\rightarrow\mathbf{Pr}^{L,\otimes-t,rc}$$
%\item
%$$F:\mathbf{QCoh}^{R}\rightarrow\mathbf{Sp(\mathbf{Ab(Str_{\big\slash(-)})})}\circ\mathcal{O}$$
%is a natural equivalence of functors $\mathbf{Aff}\rightarrow\mathbf{Cat}$.
\end{enumerate}
\end{defn}

We should explain the general idea here. $\mathbf{Aff}$ should be thought of as our category of (affine) algebro-geometric spaces. $\mathbf{Str}$ assigns to such a space $X$, the category of algebro-geometric structures on the underlying space of $X$ which receive a map from $X$. $\mathcal{O}$ should be thought of as the structure sheaf functor, and $\mathrm{Spec}$ the spectrum functor. The natural equivalence $\eta$ says that $\mathbf{Str}(X)$ is anti-equivalent to a full subcategory of affine spaces over $X$. $\mathbf{Mod}(X)$ is a category of sheaves of modules on $X$, and $\mathrm{sqz}$ is a `square-zero extension functor'.

Given $X\in\mathbf{Aff}$ we denote by $X[-]:\mathbf{Mod}(X)^{op}\rightarrow{}_{X\big\backslash}\mathbf{Aff}$ the composition $\mathrm{Spec}\circ\mathrm{sqz}$. 

Given the partial data $(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$ we can construct a pre-$(\infty,1)$-algebro-geometric tuple as follows. For $X\in\mathbf{Aff}$ we define
$$\mathbf{Mod}(X)\defeq\mathbf{Sp}(\mathbf{Ab}(\mathbf{Str}(X))$$
Let $f:X\rightarrow Y$ be map in $\mathbf{Aff}$. By assumption we get a functor
$$f_{*}:\mathbf{Str}(X)\rightarrow\mathbf{Str}(Y)$$
and an induced limit-preserving and accessible functor
$$f_{*}:\mathbf{Mod}(X)\rightarrow\mathbf{Mod}(Y)$$
In particular this functor has a left adjoint, and we get a functor
$$\mathbf{Mod}:\mathbf{Aff}\rightarrow\mathbf{Cat}^{\mathbf{R},acc,t,c,e}$$
The \textit{square-zero extension functor}
$$X[-]:\mathbf{Mod}(X)^{op}\rightarrow{}_{X\big\backslash}\mathbf{Aff}$$
is the composite
\begin{align*}
\xymatrix{
\mathbf{Sp(Ab(Str}(X)))\ar[r]^{\Omega^{\infty}}&\mathbf{Ab(Str}(X))\ar[r]^{\;\;\;\;\;U} & \mathbf{Str}(X)
}
\end{align*}
where $U$ is the forgetful functor. When we refer to the `pre-$(\infty,1)$-algebro-geometric tuple $(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$' we mean the tuple constructed in the above manner. 



%
%If $\mathbf{Aff}$ has a terminal object $\bullet$ we write $\Gamma$ for both of the functors
%$$pt_{*}:\mathbf{Str}(X)\rightarrow\mathbf{Str}(\bullet)$$
%$$pt_{*}:\mathbf{Mod}(X)\rightarrow\mathbf{Mod}(\bullet)$$
%where $pt:X\rightarrow\bullet$ is the unique map.

%\begin{defn}
%A pre-$(\infty,1)$-algebro-geometric tuple 
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{Mod},\mathrm{sqz})$$ 
%is said to be \textit{left adjointable} if $\mathbf{Mod}$ defines a functor
%$$\mathbf{Mod}:\mathbf{Aff}\rightarrow\mathbf{Cat}^{R}$$
%\end{defn}
%nd $\mathcal{Y}\in\mathbf{Str}(X)$, we define
%$$\mathbf{QCoh}(\mathcal{Y})\defeq\mathbf{Sp}(\mathbf{Ab}(\mathbf{Str}(X)_{\big\slash(\mathcal{Y})}))$$
%In particular we define
%$$\mathbf{QCoh}(X)\defeq\mathbf{QCoh}(\mathcal{O}_{X})$$



%\begin{example}
%\begin{enumerate}
%\item
%Let $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ be a spectral algebraic pre-context. Define $\mathbf{Str}$ to be the functor which sends $R$ to $\mathbf{Comm}(\mathbf{Mod}^{\le0})_{\big\slash R}$. $\mathcal{O}$ sends $R^{op}\rightarrow S^{op}$ to $S\rightarrow R$, and $\mathrm{Spec}$ sends $S\rightarrow R$ to $R^{op})\rightarrow S^{op}$. $\mathbf{QCoh}:\mathbf{Aff}\rightarrow\mathbf{Cat}$ is equivalent to the assignment $R^{op}\mapsto{}_{R}\mathbf{Mod}$.
%
%%There is an equivalence $\mathbf{QCoh}\cong\mathbf{Sp(\mathbf{Ab(Str_{\big\slash(S)})})}\circ\mathcal{O}$.
%\item
%There is a stable version of the first example in which ${}_{R}\mathbf{Mod}^{\le0}$ is replaced by ${}_{R}\mathbf{Mod}$. Again $\mathbf{QCoh}:\mathbf{Aff}\rightarrow\mathbf{Cat}$ is equivalent to the assignment $R^{op}\mapsto{}_{R}\mathbf{Mod}$.
%\item
%Let $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ be a derived algebraic context. The first two examples can be repeated, replacing $\mathbf{Comm}$ by $\mathbf{DAlg}$. 
%\item
%Let $\mathbf{R}$ be a geometric category of connective decorated rings  in a derived algebraic context $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ as in \cite{kelly2021analytic} Definition 10.10. An object of such a category is, essentially, a pair $(R,\mathbf{M}_{R})$, where $R\in\mathbf{DAlg}^{cn}(\mathbf{C})$ and $\mathbf{M}_{R}$ is a reflective subcategory of ${}_{R}\mathbf{Mod}(\mathbf{C})$. We define $\mathbf{Aff}\defeq\mathbf{R}^{op}$. Define $\mathbf{Str}$ to be the functor which sends $R$ to $\mathbf{R}_{\big\slash R}$. $\mathcal{O}$ sends $R^{op}\rightarrow S^{op}$ to $S\rightarrow R$, and $\mathrm{Spec}$ sends $S\rightarrow R$ to $R^{op}\rightarrow S^{op}$. $\mathbf{QCoh}(R^{op})$ is equivalent to $\mathbf{M}_{R}$.
%\item
%Let $\mathcal{T}$ be a pregeometry in the sense of \cite{lurie2009derived} 3.1.1. Define $\mathbf{Aff}\defeq{}^{L}\mathbf{Top}(\mathcal{T})$ to be the category of $\mathcal{T}$-structured spaces. $\mathbf{Str}$ sends $(\mathcal{X},\mathcal{O}_{X})$ to $\mathbf{Str}^{loc}_{\mathcal{T}}(\mathcal{X})_{\big\slash\mathcal{O}_{X}}$. $\mathcal{O}$ sends $(f,f^{\#}):(X,\mathcal{O}_{X})\rightarrow(Y,\mathcal{O}_{Y})$ to $f^{\#}:f^{-1}\mathcal{O}_{Y}\rightarrow\mathcal{O}_{X}$. $\mathrm{Spec}$ sends $\tilde{\mathcal{O}}_{X}\in\mathbf{Str}^{loc}_{\mathcal{T}}(\mathcal{X})_{\big\slash\mathcal{O}_{X}}$ to the natural map $(\mathcal{X},\mathcal{O}_{X})\rightarrow (\mathcal{X},\tilde{\mathcal{O}}_{X})$. We will return to this class of examples later.
%%\item
%%Again let $\mathcal{T}$ be a pregeometry in the sense of \cite{lurie2009derived} and let $\mathcal{X}$ be an $\infty$-topos. Define $\mathbf{Aff}\defeq\mathbf{Str}^{loc}_{\mathcal{T}}(\mathcal{X})$ and $\mathbf{Str},\mathcal{O},\mathrm{Spec}$ to be the restrictions to $\mathbf{Str}^{loc}_{\mathcal{T}}(\mathcal{X})\subset{}^{L}\mathbf{Top}(\mathcal{T})$.
%\end{enumerate}
%\end{example}

\begin{example}
Let $(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$ be a pre-$(\infty,1)$-algebro-geometric context and let $X\in\mathbf{Aff}$. Let $\mathbf{Aff}(X)$ denote the essential image of   $\mathrm{Spec}_{X}:\mathbf{Str}(X)\rightarrow{}_{X\big\backslash}\mathbf{Aff}^{op}$. Then
$$(\mathbf{Aff}(X),\mathbf{Str}|_{\mathbf{Aff}(X)^{op}},\mathbf{Mod}|_{\mathbf{Aff}(X)^{op}},\mathcal{O},\mathrm{Spec}_{X},\eta,\mathrm{sqz})$$
determines a pre-$(\infty,1)$-algebro-geometric context.
\end{example}
Write $\mathbf{Str}^{*}$ and $\mathbf{Mod}^{*}$ for the functors $\mathbf{Aff}^{op}\rightarrow\mathbf{Cat}$ corresponding to taking left adjoints. For a map $f:X\rightarrow Y$ in $\mathbf{Aff}$ the functor ${}_{X\big\backslash}\mathbf{Aff}^{op}\rightarrow{}_{Y\big\backslash}\mathbf{Aff}^{op}$ also has a left adjoint, corresponding to taking pullbacks. We denote by ${}_{(-)^{*}\big\backslash}\mathbf{Aff}^{op}:\mathbf{Aff}^{op}\rightarrow\mathbf{Cat}$ the functor obtained by passing to this left adjoint.

Moreover $\mathrm{Spec}^{*}$ gives a natural transformation ${}_{(-)^{*}\big\backslash}\mathbf{Aff}^{op}\rightarrow\mathbf{Str}^{*}$ and $\mathcal{O}^{*}$ a natural transformation $\mathbf{Str}^{*}\rightarrow{}_{(-)^{*}\big\backslash}\mathbf{Aff}^{op}$. $\eta$ induces a natural equivalence $\eta^{*}$ between $\mathrm{Spec}^{*}\circ\mathcal{O}^{*}$ and the identity transformation.

\begin{defn}
\begin{enumerate}
\item
A \textit{morphism of pre-}$(\infty,1)$-\textit{algebro-geometric tuples} from 
$$(\mathbf{Aff}_{\mathcal{U}},\mathbf{Str}_{\mathcal{U}},\mathcal{O}_{\mathcal{U}},\mathrm{Spec}_{\mathcal{T}},\eta_{\mathcal{U}},\mathbf{Mod}_{\mathcal{U}},\mathrm{sqz}_{\mathcal{U}})$$ 
to a pre-$(\infty,1)$-algebro-geometric tuple
$$(\mathbf{Aff}_{\mathcal{T}},\mathbf{Str}_{\mathcal{T}},\mathcal{O}_{\mathcal{T}},\mathrm{Spec}_{\mathcal{U}},\eta_{\mathcal{T}},\mathbf{Mod}_{\mathcal{T}},\mathrm{sqz}_{\mathcal{T}}))$$ 
is a tuple
$$(G,\phi,\psi,\zeta)$$
where 
\begin{enumerate}
\item
$G:\mathbf{Aff}_{\mathcal{U}}\rightarrow\mathbf{Aff}_{\mathcal{T}}$ is a functor.
\item
$\phi_{X}:\mathbf{Str}_{\mathcal{U}}(X)\rightarrow\mathbf{Str}_{\mathcal{T}}\circ G(X)$ is a collection of functors for each $X\in\mathbf{Aff}_{\mathcal{U}}$
\item
$\psi_{X}:\mathbf{Mod}_{\mathcal{U}}(X)\rightarrow\mathbf{Mod}_{\mathcal{U}}\circ G(X)$ is a collection of functors for each $X\in\mathbf{Aff}_{\mathcal{U}}$.
%\item
%Consider the diagram
%\begin{displaymath}
%\xymatrix{
%\mathbf{Str}_{\mathcal{U}}\ar[d]^{\mathrm{Spec}_{\mathcal{U}}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}\circ G\ar[d]^{\mathrm{Spec}_{\mathcal{T}}\circ G}\\
%{}_{(-)\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[r]^{G(-)} & {}_{G(-)\big\backslash}\mathbf{Aff}_{\mathcal{T}}
%}
%\end{displaymath}
%$\delta$ is a natural isomorphism $\mathrm{Spec}_{\mathcal{T}}\circ G\circ\phi\cong G(-)\circ\mathrm{Spec}_{\mathcal{U}}$
%\item
%Consider the diagram
%\begin{displaymath}
%\xymatrix{
%{}_{(-)\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[r]^{G(-)}\ar[d]^{\mathcal{O}_{\mathcal{U}}} & {}_{G(-)\big\backslash}\mathbf{Aff}_{\mathcal{T}}\ar[d]^{\mathcal{O_{\mathcal{T}}}}\\
%\mathbf{Str}_{\mathcal{U}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}\circ G(-)
%}
%\end{displaymath}
%$\epsilon$ is a natural isomorphism $\phi\circ\mathcal{O}_{\mathcal{U}}\rightarrow\mathcal{O_{\mathcal{T}}}\circ G(-)$
\item
Consider the diagram
\begin{displaymath}
\xymatrix{
\mathbf{Mod}_{\mathcal{U}}\ar[d]^{\mathrm{sqz}_{\mathcal{U}}}\ar[r]^{\psi} & \mathbf{Mod}_{\mathcal{}}\circ G\ar[d]^{\mathrm{sqz}_{\mathcal{T}}}\\
\mathbf{Str}_{\mathcal{U}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}T
}
\end{displaymath}
$\zeta$ is a natural transformation (not necessarily isomorphism!) $\mathrm{sqz}_{\mathcal{T}}\circ\psi\Rightarrow\phi\circ\mathrm{sqz}_{\mathcal{U}}$.
\end{enumerate}
Note that in general we do not assume that $\phi_{X}$ or $\psi_{X}$ assemble into natural transformations.
\item
A morphism of pre-$(\infty,1)$-algebro-geometric tuples is said to be \textit{left adjointable} if
\begin{enumerate}
\item
  each 
 $$\phi_{X}:\mathbf{Str}_{\mathcal{U}}\rightarrow\mathbf{Str}_{\mathcal{T}}\circ G$$
 is an accessible right adjoint.
 \item
each
$$\phi_{X}:\mathbf{Mod}_{\mathcal{U}}(X)\rightarrow\mathbf{Mod}_{\mathcal{T}}(G(X))$$
is an accessible right adjoint.
\end{enumerate}
\item
A morphim of pre-$(\infty,1)$-algebro-geometric tuples is said to be \textit{strongly left adjointable} if 
\begin{enumerate}
\item
it is left adjointable
\item
$G$ commutes with colimits.
\item
$\zeta$ is a natural isomorphism
\end{enumerate}
\item
A \textit{fully extended} morphim of pre-$(\infty,1)$-algebro-geometric tuples is a tuple $(G,\phi,\psi,\delta,\epsilon,\zeta)$ such that the following conditions hold
\begin{enumerate}
\item
$(G,\phi,\delta,\zeta)$ is a morphism of pre-$(\infty,1)$-algebro-geometric tuples.
\item
$\phi$ and $\psi$ extend to natural transformations
 $$\phi:\mathbf{Str}_{\mathcal{U}}\rightarrow\mathbf{Str}_{\mathcal{T}}\circ G$$
  $$\psi:\mathbf{Mod}_{\mathcal{U}}\rightarrow\mathbf{Mod}_{\mathcal{T}}\circ G$$
  \item
Consider the diagram
\begin{displaymath}
\xymatrix{
\mathbf{Str}_{\mathcal{U}}\ar[d]^{\mathrm{Spec}_{\mathcal{U}}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}\circ G\ar[d]^{\mathrm{Spec}_{\mathcal{T}}\circ G}\\
{}_{(-)\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[r]^{G(-)} & {}_{G(-)\big\backslash}\mathbf{Aff}_{\mathcal{T}}
}
\end{displaymath}
$\delta$ is a natural isomorphism $\mathrm{Spec}_{\mathcal{T}}\circ G\circ\phi\cong G(-)\circ\mathrm{Spec}_{\mathcal{U}}$
\item
Consider the diagram
\begin{displaymath}
\xymatrix{
{}_{(-)\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[r]^{G(-)}\ar[d]^{\mathcal{O}_{\mathcal{U}}} & {}_{G(-)\big\backslash}\mathbf{Aff}_{\mathcal{T}}\ar[d]^{\mathcal{O_{\mathcal{T}}}}\\
\mathbf{Str}_{\mathcal{U}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}\circ G(-)
}
\end{displaymath}
$\epsilon$ is a natural isomorphism $\phi\circ\mathcal{O}_{\mathcal{U}}\rightarrow\mathcal{O_{\mathcal{T}}}\circ G(-)$
\end{enumerate}
\item
A morphism of pre-$(\infty,1)$-algebro-geometric tuples is said to be \textit{right adjointable} if
\begin{enumerate}
\item
  each 
 $$\phi_{X}:\mathbf{Str}_{\mathcal{U}}\rightarrow\mathbf{Str}_{\mathcal{T}}\circ G$$
 is a left adjoint.
 \item
each
$$\phi_{X}:\mathbf{Mod}_{\mathcal{U}}(X)\rightarrow\mathbf{Mod}_{\mathcal{T}}(G(X))$$
is a left adjoint.
\end{enumerate}
\item
An \textit{extended right adjointable morphism} of pre-$(\infty,1)$-algebro-geometric tuple is a tuple $(G,\phi,\psi,\zeta)$ where
\begin{enumerate}
\item
$(G,\phi,\psi,\zeta)$ is a right adjointable morphism of pre-$(\infty,1)$-algebro-geometric tuple.
\item
$\phi$ and $\psi$ extend to natural transformations
$$\phi:(\mathbf{Str}^{*}_{\mathcal{U}})\rightarrow\mathbf{Str}^{*}_{\mathcal{T}}\circ G$$
$$\psi:\mathbf{Mod}^{*}_{\mathcal{U}}\rightarrow\mathbf{Mod}^{*}_{\mathcal{T}}\circ G$$
%  \item
%Consider the diagram
%\begin{displaymath}
%\xymatrix{
%\mathbf{Str}_{\mathcal{U}}\ar[d]^{\mathrm{Spec}_{\mathcal{U}}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}\circ G\ar[d]^{\mathrm{Spec}_{\mathcal{T}}\circ G}\\
%{}_{(-)\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[r]^{G(-)} & {}_{G(-)\big\backslash}\mathbf{Aff}_{\mathcal{T}}
%}
%\end{displaymath}
%$\delta$ is a natural isomorphism $\mathrm{Spec}_{\mathcal{T}}\circ G\circ\phi\cong G(-)\circ\mathrm{Spec}_{\mathcal{U}}$
%\item
%Consider the diagram
%\begin{displaymath}
%\xymatrix{
%{}_{(-)\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[r]^{G(-)}\ar[d]^{\mathcal{O}_{\mathcal{U}}} & {}_{G(-)\big\backslash}\mathbf{Aff}_{\mathcal{T}}\ar[d]^{\mathcal{O_{\mathcal{T}}}}\\
%\mathbf{Str}_{\mathcal{U}}\ar[r]^{\phi} & \mathbf{Str}_{\mathcal{T}}\circ G(-)
%}
%\end{displaymath}
%$\epsilon$ is a natural isomorphism $\phi\circ\mathcal{O}_{\mathcal{U}}\rightarrow\mathcal{O_{\mathcal{T}}}\circ G(-)$
\end{enumerate}
\end{enumerate}
\end{defn}





\begin{example}
Let
$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{Mod},\mathrm{sqz})$$
be a pre-$(\infty,1)$-algebro-geometric tuple where $\mathbf{Aff}$ has a terminal object $\bullet$. Consider the tuple
$$(\mathbf{Aff}(\bullet),\mathbf{Str}|_{\mathbf{Aff}(\bullet)},\mathbf{Mod}|_{\mathbf{Aff}(\bullet)},\mathcal{O},\mathrm{Spec},\eta,\mathrm{sqz})$$ 
We have the functor $\Gamma:\mathbf{Str}\rightarrow\mathbf{Str}(\bullet)$. We also have the composite functor
\begin{displaymath}
\xymatrix{
\mathbf{Aff}\ar[r]^{\mathcal{O}}&\mathbf{Str}^{op}(\bullet)\ar[r]^{\mathrm{Spec}}&\mathbf{Aff}(\bullet)
}
\end{displaymath}
This determines a (strongly left adjointable) morphism of pre-$(\infty,1)$-algebro-geometric tuples which can also be made fully extendable., We will also denote this transformation by $\Gamma$. 
\end{example}

Let
$$(\mathbf{Aff}_{\mathcal{U}},\mathbf{Str}_{\mathcal{U}},\mathcal{O}_{\mathcal{U}},\mathrm{Spec}_{\mathcal{U}},\eta_{\mathcal{U}})$$
and
$$(\mathbf{Aff}_{\mathcal{T}},\mathbf{Str}_{\mathcal{T}},\mathcal{O}_{\mathcal{T}},\mathrm{Spec}_{\mathcal{T}},\eta_{\mathcal{T}})$$
be partial data inducing pre-$(\infty,1)$-geometry tuples. Suppose we are also given the partial data of a morphism $(G,\phi)$, and that each $\phi_{X}$ is an accessible right adjoint. Then by stabilisation we get a right adjoint functor 
$$\psi_{X}:\mathbf{Mod}_{\mathcal{U}}(X)\rightarrow\mathbf{Mod}_{\mathcal{T}}\circ G(X)$$

Moreover, exactly as in \cite{PYYrepresentability} Proposition 5.19 we have a commutative diagram

\begin{displaymath}
\xymatrix{
\mathbf{Sp(Ab(Str_{\mathcal{U}}}(X)))\ar[d]\ar[r]^{\Omega^{\infty}}&\mathbf{Ab(Str_{\mathcal{U}}}(X))\ar[r]^{\;\;\;\;\;U}\ar[d] & \mathbf{Str_{\mathcal{U}}}(X)\ar[d]\ar[r]^{\mathrm{Spec}} &{}_{X\big\backslash}\mathbf{Aff}_{\mathcal{U}}\ar[d]\\
\mathbf{Sp(Ab(Str_{\mathcal{T}}}(X)))\ar[r]^{\Omega^{\infty}}&\mathbf{Ab(Str_{\mathcal{T}}}(X))\ar[r]^{\;\;\;\;\;U} & \mathbf{Str_{\mathcal{T}}}(X)\ar[r]^{\mathrm{Spec}} &{}_{X\big\backslash}\mathbf{Aff}_{\mathcal{T}}
}
\end{displaymath}

This gives us our $\zeta_{X}$, which is a natural isomorphism. If $(G,\phi,\delta)$ is the partial data of a fully extended morphism, then it is also possible to canonically extend this to a fully extended morphism $(G,\phi,\psi,\delta,\epsilon,\zeta)$. 

%Let $(G,\phi,\delta,\epsilon)$ be a right morphism of pre-$(\infty,1)$-algebro-geometric tuples, and let $X\in\mathbf{Aff}_{\mathcal{U}}$. 
%
%We get a functor
%$$\phi(X):\mathbf{Str}_{\mathcal{U}}(X)\rightarrow\mathbf{Str}_{\mathcal{T}}(G(X))$$
%and an induced functor
%$$\phi(X):\mathbf{Mod}_{\mathcal{U}}(X)\rightarrow\mathbf{Mod}_{\mathcal{T}}(G(X))$$
%
%
%
%If a morphism is left adjointable then it is stably left adjointable. Indeed, the induced functor
%$$\phi(X):\mathbf{Mod}_{\mathcal{U}}(X)\rightarrow\mathbf{Mod}_{\mathcal{T}}(G(X))$$
%is an accessible functor which commutes with limits, and is therefore a right adjoint functor.
%is accessible and commutes with limits, so we get an adunction
%$$\adj{\psi(X)}{\mathbf{QCoh}_{\mathcal{T}}(G(X))}{\mathbf{QCoh}_{\mathcal{U}}(X)}{\phi(X)}$$
%and for each $\mathcal{Y}\in\mathbf{Str'}(G(X))$ an induced adjunction
%$$\adj{\phi(X)_{\mathcal{Y}}}{\mathbf{Str}(X)_{\big\slash\psi(X)(\mathcal{Y})}}{\mathbf{Str'}(G(X))_{\big\slash\mathcal{Y}}}{\psi(X)_{\mathcal{Y}}}$$
%The induced functor 
%$$\psi^{st}(X):\mathbf{QCoh}'(\mathcal{Y})\rightarrow\mathbf{QCoh}(\psi(X)(\mathcal{Y}))$$
%is accessible and commutes with limits, so we get an adjunction
%$$\adj{\phi^{st}(X)_{\mathcal{Y}}}{\mathbf{QCoh}(\psi(X)(\mathcal{Y}))}{\mathbf{QCoh}'(\mathcal{Y})}{\psi^{st}(X)_{\mathcal{Y}}}$$

%Let $f:\mathbb{X}\rightarrow\mathbb{Y}$ be a map in $\mathbf{Str}(X)$. We get an adjunction
%$$\adj{f^{*}}{\mathbf{Str}(X)_{\mathbb{Y}}}{\mathbf{Str}(X)_{\mathbb{X}}}{f_{*}}$$
%$f_{*}$ is accessible, and this implies the existence of an adjunction
%$$\adj{f^{*}}{\mathbf{QCoh}(\mathbb{Y})}{\mathbf{QCoh}(\mathbb{X)}}{f_{*}}$$
%More generally let $g:X\rightarrow Y$ be a map in $\mathbf{Aff}$ by assumption we get an adjunction
%$$\adj{L_{f}}{\mathbf{Str}(Y)}{\mathbf{Str}(X)}{R_{f}}$$





\subsection{The Cotangent Complex and Obstruction Theories}

In this section we show that the abstract setup of algebro-geometric tuples lends itself to a general theory of cotangent complexes and obstruction theories.

\subsubsection{The Cotangent Complex}

First we give straightforward generalisations of material from \cite{kelly2021analytic}. Fix a pre-$(\infty,1)$-algebro-geometric tuple
$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{Mod},\mathrm{sqz})$$


\begin{defn}[\cite{toen2008homotopical}, Definition 1.4.1.4]
Let $\mathcal{X}\in\mathbf{PreStk}(\mathbf{Aff})$, $Y\in\mathbf{Aff}$, and $x:Y\rightarrow\mathcal{X}$ a map. Define 
$$\mathrm{Der}_{\mathcal{X}}(\mathrm{Spec}(A),-):\mathbf{Mod}(\mathrm{Spec}(A))\rightarrow\textbf{sSet}$$
to be the functor
$$\mathrm{Map}_{{}_{Y\big\backslash\mathbf{Aff}}}(Y[M],\mathcal{X})$$
\end{defn}
A cotangent complex at $x:Y\rightarrow\mathcal{X}$ is, in principle, an object of $\mathbf{Mod}(A)$ copresenting $\mathrm{Der}_{\mathcal{X}}(\mathrm{Spec}(A),-)$. However we only expect such an object to exist with restrictions on $M$ and $A$. 



\begin{defn}
Let
\begin{enumerate}
\item
$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{Mod},\mathrm{sqz})$$
be a pre-algebro-geometric tuple. 
\item
$\mathbf{A}\subset\mathbf{Aff}$ be a full subcategory.
\item
$\tau$ be a topology on $\mathbf{Aff}$
\item
$\mathbf{P}$ be a class of maps in $\mathbf{Aff}$
\end{enumerate}
such that
$$(\mathbf{Aff},\tau,\mathbf{P},\mathbf{A})$$
is a strong relative $(\infty,1)$-geometry tuple. A \textit{good system of module categories relative to} $(\mathbf{A},\tau,\mathbf{P})$, denoted, $\mathbf{F}$ is an assignment to each $Y\in \mathbf{A}$ a full subcategory $\mathbf{F}_{Y}\subset\mathbf{Mod}(Y)$ such that
\begin{enumerate}
\item
$\mathcal{O}_{X}\in\mathbf{F}_{X}$ for any $X\in\mathbf{A}$;
\item
$\mathbf{F}_{X}$ is closed under equivalences, finite colimits, and retracts;
\item
$f^{*}M\in\mathbf{F}_{Y}$ for any map $f:Y\rightarrow X$ and any $M\in\mathbf{F}_{Y}$. 
\item
any $F\in\mathbf{F}_{A}$ satisfies weak \v{C}ech descent;
\item
For $M\in\mathbf{F}_{A}^{1}$ and $\mathrm{Spec}(A)\in\mathbf{A}$, $\mathrm{Spec}(A\oplus M)\in\mathbf{A}$. 
\end{enumerate}
\end{defn}

Moreover for each $n\in\mathbb{Z}$ we also define
$$\mathbf{F}_{X}^{\le n}\defeq\mathbf{F}_{X}\times_{\mathbf{Mod}(X)}\mathbf{Mod}(X)^{\le n}$$
$$\mathbf{F}_{X}^{cn}\defeq\mathbf{F}_{X}\times_{\mathbf{Mod}(X)}\mathbf{Mod}(X)^{cn}$$



\begin{defn}
A \textit{weak relative }$(\infty,1)$-\textit{algebro-geometric context} is a tuple
$$(\mathbf{Aff},\tau,\mathbf{P},\mathbf{A},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{Mod},\mathrm{sqz},\mathbf{F})$$
where
\begin{enumerate}
\item
$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$ is a left adjointable pre-$(\infty,1)$-algebro-geometric tuple.
\item
$(\mathbf{Aff},\tau,\mathbf{P},\mathbf{A})$ is a strong relative $(\infty,1)$-geometry tuple.
\item
$\mathbf{F}$ is a good system of module categories relative to $(\mathbf{A},\tau,\mathbf{P})$.
\end{enumerate}
\end{defn}

\begin{defn}
A morphism of weak relative $(\infty,1)$-algebro-geometric context from
$$(\mathbf{Aff}_{\mathcal{U}},\tau_{\mathcal{U}},\mathbf{P}_{\mathcal{U}},\mathbf{A}_{\mathcal{U}},\mathbf{Str}_{\mathcal{U}},\mathcal{O}_{\mathcal{U}},\mathrm{Spec}_{\mathcal{U}},\eta_{\mathcal{U}},\mathbf{F}_{\mathcal{U}})$$
to
$$(\mathbf{Aff}_{\mathcal{T}},\tau_{\mathcal{T}},\mathbf{P}_{\mathcal{T}},\mathbf{A}_{\mathcal{T}},\mathbf{Str}_{\mathcal{T}},\mathcal{O}_{\mathcal{T}},\mathrm{Spec}_{\mathcal{T}},\eta_{\mathcal{T}},\mathbf{F}_{\mathcal{T}})$$
is a left adjointable morphism $(G,\phi,\delta,\epsilon)$ of the underlying pre-$(\infty,1)$-algebro-geometric contexts such that
\begin{enumerate}
\item
$G$ determines a morphism of relative $(\infty,1)$-geometry tuples 
$$(\mathbf{Aff}_{\mathcal{U}},\tau_{\mathcal{U}},\mathbf{P}_{\mathcal{U}},\mathbf{A}_{\mathcal{U}})\rightarrow(\mathbf{Aff}_{\mathcal{T}},\tau_{\mathcal{T}},\mathbf{P}_{\mathcal{T}},\mathbf{A}_{\mathcal{T}})$$
\item
for any $A\in\mathbf{A}_{\mathcal{U}}$ and any $M\in\mathbf{F}_{\mathcal{T},\mathbf{G(A)}}$, $\phi(X)^{*}(M)\in\mathbf{F}_{\mathcal{U},G(\mathbf{A})}$. 
\end{enumerate}
\end{defn}



\begin{defn}[\cite{toen2008homotopical}, Definition 1.4.1.14]
Let $U\in\mathbf{A}$. A map $f:\mathcal{X}\rightarrow\mathcal{Y}$ in $\mathbf{PreStk}(\mathbf{Aff})$ is said to \textit{have a cotangent complex at }$x:U\rightarrow\mathcal{X}$ \textit{relative to} $\mathbf{F}$ if there is a connective $\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x}\in\mathbf{F}^{cn}_{U}$ and an equivalence 
$$\mathrm{Der}_{\mathcal{X}\big\slash\mathcal{Y}}(U,-)\cong\mathrm{Map}_{\mathbf{Mod}(U)}(\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x},-)$$
\end{defn}


In the setting of geometry relative to a weak relative $(\infty,1)$-algebro-geometric tuples it is possible to meaningfully define cotangent complexes of stacks, and tangent stacks. Here we follow \cite{toen2008homotopical} Section 1.4.1.



\begin{defn}[\cite{toen2008homotopical} Section 1.4.1]
Let $f:\mathcal{X}\rightarrow\mathcal{Y}$ be a map in $\mathbf{PreStk}(\mathbf{Aff})$ and $x:U\rightarrow\mathcal{X}$ a map. By composition we get a map
$$\mathrm{Der}_{\mathcal{X}}(U,-)\rightarrow \mathrm{Der}_{\mathcal{Y}}(U,-).$$
We define 
$$\mathrm{Der}_{\mathcal{X}\big\slash\mathcal{Y}}(U,-):\mathbf{Mod}^{\mathrm{cn}}(A)\rightarrow\textbf{sSet}$$
to be the fibre of the map $\mathrm{Der}_{\mathcal{X}}(U,-)\rightarrow \mathrm{Der}_{\mathcal{Y}}(U,-)$.
\end{defn}


\begin{defn}[\cite{toen2008homotopical}, Definition 1.4.1.14]
A map $f:\mathcal{X}\rightarrow\mathcal{Y}$ in $\mathbf{PreStk}(\mathbf{Aff})$ is said to \textit{have a cotangent complex at }$x:U\rightarrow\mathcal{X}$\textit{ relative to }$\mathbf{F}$ if there is a $(-n)$-connective $A$-module $\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x}\in\mathbf{F}_{A}$ and an equivalence 
$$\mathrm{Der}_{\mathcal{X}\big\slash\mathcal{Y}}(U,-)\cong\mathrm{Map}_{\mathbf{Mod}_{A}}(\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x},-)$$
\end{defn}



Let

\begin{displaymath}
\xymatrix{
\mathrm{Spec}(B)\ar[dr]^{y}\ar[rr]^{u} & & \mathrm{Spec}(A)\ar[dl]^{x}\\
& \mathcal{X} & 
}
\end{displaymath}
be a commutative diagram with $u$ a morphism in $\mathbf{A}$. Suppose that $f:\mathcal{X}\rightarrow\mathcal{Y}$ has a relative cotangent complex at both $x$ and $y$. Using the universal properties of $\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x}$ and $\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},y}$, there is a natural map.
$$\tilde{u}:\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},y}\rightarrow u^{*}(\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x})$$

\begin{defn}[\cite{toen2008homotopical} Definition 1.4.1.15]
A morphism $f:\mathcal{X}\rightarrow\mathcal{Y}$ of prestacks is said to have a \textit{global cotangent complex relative to }$\mathbf{A}$ if
\begin{enumerate}
\item
for any $U\in\mathbf{A}$ and any $x:U\rightarrow\mathcal{X}$, $f$ has a relative cotangent complex at $x$ 
\item
For any morphism $u:U\rightarrow V$ in $\mathbf{A}$, and any commutative diagram
\begin{displaymath}
\xymatrix{
U\ar[dr]^{y}\ar[rr]^{u} & &V\ar[dl]^{x}\\
& \mathcal{X} & 
}
\end{displaymath}
the map 
$$\tilde{u}:\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},y}\rightarrow u^{*}(\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y},x})$$
is an equivalence. 
\end{enumerate}
$f$ is said to \textit{have a global contangent complex} if it has a global cotangent complex relative to $(\mathbf{Aff},\mathbf{Mod})$.
\end{defn}

\begin{rem}
If $f:\mathcal{X}\rightarrow\mathcal{Y}$ has a global contangent complex, then this data determines an object $\mathbb{L}_{\mathcal{X}\big\slash\mathcal{Y}}\in\mathbf{Mod}(\mathcal{X})$.
\end{rem}

Let $X\in\mathbf{Aff}$ and let $M\in\mathbf{Mod}(X)^{\le -1}$. Consider the trivial square-zero extension $X[M]$, and let $d:\mathcal{O}_{X}\rightarrow \mathcal{O}_{X}\oplus M$ be a derivation. We define $X_{d}[M]$ to be $\mathrm{Spec}(\mathcal{O}_{X}\oplus_{d}M)$, where $\mathcal{O}_{X}\oplus_{d}\Omega M$ is defined by the pullback diagram below.
\begin{displaymath}
\xymatrix{
\mathcal{O}_{X}\oplus_{d}\Omega M\ar[d]\ar[r] & \mathcal{O}_{X}\oplus M\ar[d]^{i}\\
 \mathcal{O}_{X}\ar[r]^{d} &  \mathcal{O}_{X}\oplus\mathcal{F}
}
\end{displaymath}
Here $i:\mathcal{O}_{X}\rightarrow\mathcal{O}_{X}\oplus\mathcal{F}$ is the trivial derivation. 

\begin{defn}[ \cite{toen2008homotopical} Definition 1.4.2.1]
\begin{enumerate}
\item
A pre-stack $\mathcal{X}\in\mathbf{PreStk}(\mathbf{Aff}^{cn}_{\mathbf{C}})$ is said to be \textit{inf-cartesian relative to }$\mathbf{A}$ if for any $A$ with $\mathrm{Spec}(A)\in\mathbf{A}$, any $1$-connective $M\in\mathbf{F}^{1}_{\mathbf{A}}$, and any derivation $d\in\pi_{0}\mathrm{Der}(A,M)$, the square 
\begin{displaymath}
\xymatrix{
\mathcal{X}(A\oplus_{d}\Omega M)\ar[d]\ar[r] & \mathcal{X}(A)\ar[d]^{d}\\
\mathcal{X}(A)\ar[r]^{s} & \mathcal{X}(A\oplus M)
}
\end{displaymath}
is cartesian in $\textbf{sSet}$.
\item
A pre-stack $\mathcal{X}$ \textit{has an obstruction theory relative to }$\mathbf{A}$ if it has a global cotangent complex relative to $\mathbf{A}$, and it is inf-cartesian relative to $\mathbf{A}$.
\end{enumerate}
\end{defn}

\begin{prop}[\cite{kelly2021analytic}, Proposition 8.12]
Let $f:\mathcal{X}\rightarrow\mathcal{Y}$ be a representable map in $\mathbf{Stk}(\mathbf{A},\tau|_{\mathbf{A}},\mathbf{P}|_{\mathbf{A}})$. Then $f$ has an obstruction theory relative to $\mathbf{A}$.
\end{prop} 

\subsubsection{Lifting Maps}

\begin{defn}
Let 
$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$$ 
be a pre-$(\infty,1)$-algebro-geometric tuple, and let $X\in\mathbf{Aff}$. We define $t^{\ge -n}X$ to be
$$t^{\ge -n}X\defeq\mathrm{Spec}(\tau^{\le -n}\mathcal{O}_{X})$$
\end{defn}

Note that there are compatible maps 
$$t^{\ge -n}X\rightarrow t^{\ge -n-1}\rightarrow X$$

\begin{defn}
\begin{enumerate}
\item
$X$ is said to \textit{have a convergent Postnikov tower} if the map
$$\colim t^{\ge -n}X\rightarrow X$$
is an equivalence. 
\item
$X$ is said to have a \textit{constructibly convergent Postnikov tower} if it has a convergent Postnikov tower and there exists a derivation
$$d:\mathbb{L}_{\tau^{\ge -n}\mathcal{O}_{X}}\rightarrow\pi_{-n-1}(\mathcal{O}_{X})[n+2]$$
such that the square
%\xymatrix{
%\tau^{\le -n-1}\mathcal{O}_{X}\ar[d]\ar[r] & \tau^{\le -n}\mathcal{O}_{X}\ar[d]^{\eta_{d}}\\
%\tau^{\le -n}\mathcal{O}_{X}\ar[r]^{\eta_{0}\;\;\;\;\;\;} & \tau^{\le -n}\mathcal{O}_{X}\oplus\pi^{-n-1}(\mathcal{O}_{X})[n+2]
%}
%\end{displaymath}
\begin{displaymath}
\xymatrix{
t_{\le n}Y[\pi_{n+1}(\mathcal{O}_{Y})[n+2]]\ar[d]\ar[r] & t_{\le n}Y\ar[d]\\
t_{\le n}Y\ar[r] & t_{\le n+1}Y
}
\end{displaymath}
is a pushout
\end{enumerate}
\end{defn}


%
%Let $\mathcal{T}$ be a pregeometry. Fix a full subcategory $\mathbf{dAff}\subset{}^{L}\mathbf{Top}(\mathcal{T})$, and for each $X\in\mathbf{dAff}$ a full subcategory $\mathbf{F}_{X}\subset{}_{\mathcal{O}_{X}}\mathbf{Mod}$ such that
%\begin{enumerate}
%\item
%For each $X\in\mathbf{dAff}$ and each $n\in\mathbb{N}_{0}$ we have $\pi_{0}(X)\in\mathbf{F}_{X}$
%\item
%For each $f:X\rightarrow X'$ in $\mathbf{dAff}$ and each $\mathcal{F}\in\mathbf{F}_{X'}$ we have $f^{*}\mathcal{F}\in\mathbf{F}_{X}$.
%\end{enumerate}
%
%We denote by $\mathbf{F}^{-1}_{X}$ the full subcategory of $\mathbf{F}_{X}$ consisting of $-1$-coconnective objects




\begin{defn}
\cite{porta}
$\mathcal{Y}\in\mathbf{PreStk}(\mathbf{Aff})$ is said to \textit{have an obstruction theory relative to} $(\mathbf{A},\mathbf{F})$ if
\begin{enumerate}
%\item
%For each $n$ there exists a derivation
%$$d:\mathbb{L}^{\mathcal{U}}_{\tau_{\le n}\mathcal{O}_{X}}\rightarrow\pi_{n+1}(\mathcal{O}_{X})[n+2]$$ such that the square
%\begin{displaymath}
%\xymatrix{
%\tau_{\le n+1}\mathcal{O}_{X}\ar[d]\ar[r] & \tau_{\le n}\mathcal{O}_{X}\ar[d]^{\eta_{d}}\\
%\tau_{\le n}\mathcal{O}_{X}\ar[r]^{\eta_{0}} & \tau_{\le n}\mathcal{O}_{X}\oplus\pi_{n+1}(\mathcal{O}_{X})[n+2]
%}
%\item
%\end{displaymath}
%is a pullback.
\item
$\mathbf{Y}$ has a connective cotangent complex relative to $(\mathbf{A},\mathbf{F})$ if
\item
For any $X\in\mathbf{A}$ and any $M\in\mathbf{F}^{\le-1}_{X}$ and any derivation $d:\mathcal{O}_{X}\rightarrow\mathcal{F}$ the square
\begin{displaymath}
\xymatrix{
\mathbf{Map}(X_{d}[M],\mathcal{Y})\ar[d]\ar[r] & \mathbf{Map}(X[M],\mathcal{Y})\ar[d]\\
\mathbf{Map}(X[M],\mathcal{Y})\ar[r] & \mathbf{Map}(X,\mathcal{Y})
}
\end{displaymath}
is a pullback square. 
\end{enumerate}
\end{defn}

Exactly as in \cite{toen2008homotopical} Proposition 1.4.2.5 one can prove the following.

\begin{prop}
Let $\mathcal{Y}$ be a stack which has an obstruction theory relative to $(\mathbf{A},\mathbf{F})$. Let $X\in\mathbf{A}$, $M\in\mathbf{F}^{\le-1}_{X}$, $d:\mathcal{O}_{X}\rightarrow M$ a derivation, and $f:X\rightarrow \mathcal{Y}$ a map. Then
\begin{enumerate}
\item
There exists a natural obstruction
$$\alpha(f)\in\pi_{0}(\mathbf{Map}_{{}_{\mathbf{Mod}(X)}}(f^{*}\mathbb{L}_{F},M))$$
which vanishes if and only if the fibre of the map
$$\mathbf{Map}(X_{d}[\Omega M],F)\rightarrow\mathbf{Map}(X,F)$$
at $f$ is non-empty.
\item
If $\alpha(f)=0$ then there is a non-canonical equivalence
$$\mathbf{Map}_{X\big\slash\mathbf{Aff}}(X_{d}[\Omega M],F)\cong\Omega\mathbf{Map}_{\mathbf{Mod}(X)}(f^{*}\mathbb{L}_{F},M)$$
\end{enumerate}
\end{prop}

\begin{defn}
Let $F$ be a stack and $M\in{}_{\mathcal{O}_{F}}\mathbf{Mod}^{\mathcal{T}}$. $M$ is said to be \textit{projective in tor-amplitude }$0$\textit{ relative to }$\mathbf{A}$ if for any $n\in\mathbb{N}_{0}$, any $X\in\mathbf{A}$ such that $t_{\le n}X\rightarrow X$ is an equivalence, and any map $f:X\rightarrow F$, one has that 
$$\mathbf{Map}(f^{*}M,N)\cong 0$$
for any $N\in\mathbf{Mod}(X)^{\ge -n}$.
\end{defn}

\begin{cor}
Let $F$ be a stack which has an obstruction theory relative to $(\mathbf{A},\mathbf{F})$ and $f:X\rightarrow F$ a map with $X\in\mathbf{A}$. Suppose that  $\mathbb{L}_{F}$ is projective in tor-amplitude $0$ relative to $\mathbf{dAff}$.
%\begin{enumerate}
%\item
%\item
%the $t$-structure on  ${}_{\mathcal{O}_{X}}\mathbf{Mod}^{\mathcal{T}}$ is left complete. 
%\end{enumerate}
Then for any $M\in\mathbf{F}_{X}^{\le-n-1}$ and any derivation $d:\mathcal{O}_{X}\rightarrow M$ there is a unique lift of $f$ to a map
$$X_{d}[\Omega M]\rightarrow F$$
\end{cor}

% For each $n\ge0$ \textcolor{red}{fix:check co/homological grading}. We define 
%$$t_{\le n}X\defeq(\mathcal{X},\tau_{\le n}\mathcal{O}_{X})$$
%For each $n$ we have natural maps
%$$t_{\le n}X\rightarrow t_{\le n+1}X\rightarrow X$$



\begin{cor}
Let $\mathcal{Y}$ be a stack which has an obstruction theory relative to $(\mathbf{A},\mathbf{F})$ and $f:X\rightarrow \mathcal{Y}$ a map with $X\in\mathbf{A}$.  Suppose that
\begin{enumerate}
\item
$\mathbb{L}_{\mathbf{Y}}$ is projective and in tor-amplitude $0$ relative to $(\mathbf{A},\mathbf{F})$.
\item
$X$ has a constructible convergent Postnikov tower. 
\end{enumerate}
Then any map $t_{0}(X)\rightarrow Y$ admits a unique lift to a map $X\rightarrow Y$. 
\end{cor}







%Let $(G,\phi_{L},\delta,\epsilon)$ be a morphism from a pre-$(\infty,1)$-algebro-geometric tuple
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{QCoh},\mathbf{F})$$ 
%to a pre-$(\infty,1)$-algebro-geometric tuple
%$$(\mathbf{Aff}',\mathbf{Str}',\mathcal{O}',\mathrm{Spec}',\eta',\mathbf{QCoh}',\mathbf{F}')$$
%Suppose that $\mathbf{Aff}$ has a terminal object. We consider the functor

 
%and let $X\in\mathbf{Aff}$. Suppose further that $\phi_{L}:\mathbf{Str}\rightarrow\mathbf{Str'}\circ G$ has an accessible right adjoint $\phi_{R}$. For $X\in\mathbf{Aff}'$ we get an adjunction
%$$\adj{\phi_{L}^{stab}}{\mathbf{QCoh}(\phi_{R}(X))}{\mathbf{QCoh}'(X)}{\phi_{R}^{stab}}$$
%Suppose further that whenever $X\in\mathbf{Aff}'$ and $M\in\mathbf{F}_{\phi_{R}(X)}$, then $\phi_{L}^{stab}(M)\in\mathbf{F}'_{X}$. 
%\textcolor{red}{fix:make this into definition}
%
%\textcolor{red}{fix:put this in first, second sections}
%Let 
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{QCoh},F)$$ 
%be a pre-$(\infty,1)$-algebro-geometric tuple and let $\mathbf{S}\subset\mathbf{Aff}$ be a full-subcategory. 

\subsection{Comparison Results}

 Let $(G,\phi,\psi,\delta,\epsilon)$ be a morphism from a pre-$(\infty,1)$-algebro-geometric tuple
$$(\mathbf{Aff}_{\mathcal{U}},\mathbf{Str}_{\mathcal{U}},\mathcal{O}_{\mathcal{U}},\mathrm{Spec}_{\mathcal{U}},\eta_{\mathcal{U}},\mathbf{Mod}_{\mathcal{U}},\mathbf{F}_{\mathcal{U}})$$ 
to a pre-$(\infty,1)$-algebro-geometric tuple
$$(\mathbf{Aff}_{\mathcal{T}},\mathbf{Str}_{\mathcal{T}},\mathcal{O}_{\mathcal{T}},\mathrm{Spec}_{\mathcal{T}},\eta_{\mathcal{T}},\mathbf{Mod}_{\mathcal{T}},\mathbf{F}_{\mathcal{T}})$$ 
We wish to investigate when $G$ restricts to a fully faithful functor on subcategories of $\mathbf{Aff}_{\mathcal{U}}$. 


\subsubsection{Comparison Results for Fully Extendable, Strongly Left Adjointable Morphisms}

 The strategy for our first comparison result is based on \cite{pridham} Proposition 3.25. Modulo the increased generality the proof is the same.
 

% Fix $S\in\mathbf{Str}_{\mathcal{U}}$, and denote by $\psi(S)$ the left adjoint of $\phi(S)$. Let $\mathbf{dAff}\subset\mathbf{dSpace}\subset\mathbf{Str}_{\mathcal{T}}G(S))$ be full subcategories. We consider the functor
% $$\psi(S):\mathbf{dSpace}\rightarrow\mathbf{Str}_{\mathcal{U}}(S)$$
% and we wish to investigate when this functor is fully faithful.
 
% \begin{thm}\label{thm:generalcomparison}
% Fix full subcategories $\mathbf{dAff}\subset\mathbf{dSpace}\subset\mathbf{Aff}_{\mathcal{U}}$. Suppose that:
% 
% \begin{enumerate}
% \item
% For any $X\in\mathbf{dAff}$ and $Y\in\mathbf{dSpace}$ such that $t_{0}Y\rightarrow Y$ is an equivalence and any $X\in\mathbf{dAff}$ the map
% $$\mathbf{Map}_{\mathbf{dSpace}}(Y,X)\rightarrow\mathbf{Map}_{\mathbf{Aff}_{\mathcal{T}}}(G(Y),G(X))$$
% is an equivalence.
% \item
% For any $Y\in\mathbf{dSpace}$ both $Y$ has a constructibly convergent Postnikov towers.
% \item
% For any $Y\in\mathbf{dSpace}$ the map $\colim G(t_{\le n} Y)\rightarrow G(Y)$ is an equivalence.
%% \item
%% For any $n$ the map 
%% $$G(t_{\le n}Y[\psi(Y)(\pi_{n+1}(\mathcal{O}_{Y})[n+1])\rightarrow G(t_{\le n}Y)[\psi(\tau_{\le n}(Y))(\pi_{n+1}(\mathcal{O}_{Y}[n+1]))]$$
%%  is an equivalence.
% \item
% For any $n$ the diagram
% \begin{displaymath}
% \xymatrix{
%G (t_{\le n}Y)[\psi_{t_{\le n}(Y)}(\pi_{n+1}(\mathcal{O}_{Y}[n+1]))]\ar[d]\ar[r] & G(t_{\le n}Y)\ar[d]\\
%G(t_{\le n}Y)\ar[r] & G(t_{\le n+1}Y)
% }
% \end{displaymath}
% is a pushout diagram realising $G(t_{\le n+1}Y)$ as a square-zero extension of $G(t_{\le n}Y)$ by $\psi_{t_{\le n}(Y)}(\pi_{n+1}(\mathcal{O}_{Y}[n+1]))$. 
%  \item
% For any $X\in\mathbf{dAff}$ and $Y\in\mathbf{dSpace}$ the map
%$$\mathbf{Map}_{\mathbf{Mod}^{\mathcal{T}}(X)}(f^{*}\mathbb{L}^{\mathcal{U}}_{X},\pi_{n+1}\mathcal{O}_{Y}[n+1])\rightarrow\mathbf{Map}_{\mathbf{Mod}^{\mathcal{U}}(G(X))}(G(f)^{*}\mathbb{L}^{\mathcal{T}}_{G(X)},\psi_{t_{\le n}(Y)}(\pi_{n+1}(\mathcal{O}_{Y}[n+1])))$$
% is an equivalence.
% \end{enumerate}
% Then for any $Y\in\mathbf{dSpace}$ and any $X\in\mathbf{dAff}$ the map
% $$\mathbf{Map}_{\mathbf{dSpace}}(Y,X)\rightarrow\mathbf{Map}_{\mathbf{Aff}_{\mathcal{T}}}(G(Y),G(X))$$
% is an equivalence.
% \end{thm}
Let $(G,\phi,\psi,\delta,\epsilon)$ be a fully extended, strongly left adjointable morphism from a pre-$(\infty,1)$-algebro-geometric tuple
$$(\mathbf{Aff}_{\mathcal{U}},\mathbf{Str}_{\mathcal{U}},\mathcal{O}_{\mathcal{U}},\mathrm{Spec}_{\mathcal{U}},\eta_{\mathcal{U}},\mathbf{Mod}_{\mathcal{U}},\mathbf{F}_{\mathcal{U}})$$ 
to a pre-$(\infty,1)$-algebro-geometric tuple
$$(\mathbf{Aff}_{\mathcal{T}},\mathbf{Str}_{\mathcal{T}},\mathcal{O}_{\mathcal{T}},\mathrm{Spec}_{\mathcal{T}},\eta_{\mathcal{T}},\mathbf{Mod}_{\mathcal{T}},\mathbf{F}_{\mathcal{T}})$$ 
 An easy argument by universal properties shows that 
if $X\rightarrow Y\in\mathbf{Aff}_{\mathcal{U}}$ is such that both $X\rightarrow Y$ and $G(X)\rightarrow G(Y)$ have (connective) cotangent complexes then there is a natural map
$$\mathbb{L}_{X\big\slash Y}\rightarrow\psi^{L}_{X}(\mathbb{L}_{G(X)\big\slash G(Y)})$$
where $\psi^{L}_{X}$ is the left adjoint of $\psi_{X}$.

\begin{thm}

Let 
$$\mathbf{dAff}\subset\mathbf{dSpace}\subset\mathbf{Aff}_{\mathcal{U}}$$
 be  full subcategories. Suppose that
\begin{enumerate}
\item
For any $Y\in\mathbf{dSpace}$ such that $t_{0}Y\rightarrow Y$ is an equivalence and any $X\in\mathbf{dAff}$, the map
$$\mathbf{Map}_{\mathbf{dSpace}}(Y,X)\rightarrow\mathbf{Map}_{\mathbf{Aff}_{\mathcal{T}}}(G(X),G(Y))$$
is an equivalence.
\item
For any $X\in\mathbf{dAff}$ the map
$$\mathbb{L}_{X\big\slash Y}\rightarrow\psi^{L}_{X}(\mathbb{L}_{G(X)\big\slash G(Y)})$$
is an equivalence.
\item
Any $Y\in\mathbf{dSpace}$ has a constructibly convergent Postnikov tower.
%For any $Y\in\mathbf{dSpace}$ there exists a derivation
%$$d:\mathbb{L}^{\mathcal{U}}_{\tau_{\le n}\mathcal{O}_{Y}}\rightarrow\pi_{n+1}(\mathcal{O}_{Y})[n+2]$$ such that the square
%\begin{displaymath}
%\xymatrix{
%\tau_{\le n+1}\mathcal{O}_{Y}\ar[d]\ar[r] & \tau_{\le n}\mathcal{O}_{Y}\ar[d]^{\eta_{d}}\\
%\tau_{\le n}\mathcal{O}_{Y}\ar[r]^{\eta_{0}} & \tau_{\le n}\mathcal{O}_{Y}\oplus\pi_{n+1}(\mathcal{O}_{Y})[n+2]
%}
%\end{displaymath}
%is a pullback.
%\item
%For any $Y\in\mathbf{dSpace}$ the map
%$$\colim t_{\le n}Y\rightarrow Y$$
%is an equivalence.
\end{enumerate}
Then for any $Y\in\mathbf{dSpace}$ and any $X\in\mathbf{dAff}$ the map 
$$\mathbf{Map}_{\mathbf{dSpace}}(Y,X)\rightarrow\mathbf{Map}_{\mathbf{Aff}_{\mathcal{T}}}(G(X),G(Y))$$
is an equivalence.
\end{thm}
 
 \begin{proof}
 Since $Y$ has a constructibly convergent Postnikov tower and $\colim G(t_{\le n} Y)\rightarrow G(Y)$ is an equivalence we may assume that $t_{\le n}Y\rightarrow Y$ is an equivalence for some $n$. The proof now proceeds by induction. The case $n=0$ is by assumption. Suppose we have proven the claim for some $n$. Let $f\in\pi_{0}(\mathbf{Map}(Y,X))$.
 
 We have a fibre sequence
 \begin{displaymath}
 \xymatrix{
 \mathbf{Map}(t_{\le n+1}Y,X)_{[f]}\ar[r]&\mathbf{Map}(t_{\le n}Y,X)_{[f]}\ar[r]&\mathbf{Map}_{\mathbf{Mod}^{\mathcal{T}}(X)}(f^{*}\mathbb{L}^{\mathcal{U}}_{X},\pi_{n+1}\mathcal{O}_{Y}[n+1])
 }
 \end{displaymath}
 On the other hand applying $G$ gives a pushout square
\begin{displaymath}
\xymatrix{
G(t_{\le n}Y[\pi_{n+1}(\mathcal{O}_{Y})[n+2]])\ar[d]\ar[r] & G(t_{\le n}Y)\ar[d]\\
G(t_{\le n}Y)\ar[r] & G(t_{\le n+1}Y)
}
\end{displaymath}
Now $G(t_{\le n}Y[\pi_{n+1}(\mathcal{O}_{Y})[n+2]])\cong G(t_{\le n}Y)[\phi(Y)(\pi_{n+1}(\mathcal{O}_{Y})[n+2])]$ and this realises $G(t_{\le n+1}Y)$ as the square zero extension of $G(t_{\le n}Y)$.
%\begin{displaymath}
%\xymatrix{
%\Gamma^{\mathcal{T}}(Y,\tau_{\le n+1}\mathcal{O}_{Y})\ar[d]\ar[r] & \Gamma^{\mathcal{T}}(Y,\tau_{\le n}\mathcal{O}_{Y})\ar[d]^{\Gamma^{\mathcal{T}}(\eta_{d})}\\
%\Gamma^{\mathcal{T}}(Y,\tau_{\le n}\mathcal{O}_{Y})\ar[r]^{\Gamma^{\mathcal{T}}(\eta_{0})\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;} & \Gamma^{\mathcal{T}}(Y,\tau_{\le n}\mathcal{O}_{Y}\oplus\pi_{n+1}(\mathcal{O}_{Y})[n+2])
%}
%\end{displaymath}
Then again for $[f]\in\pi_{0}\mathbf{Map}(t_{\le0}Y,X)\cong\mathbf{Map}(G(t_{\le0}Y),G(X))$, we again get a fibre sequence
\begin{align*}
\mathbf{Map}(G(t_{\le n+1}Y),G(X))_{[f]}&\rightarrow\mathbf{Map}(G(t_{\le n}Y),G(X))_{[f]}\\
\rightarrow\mathbf{Map}_{\mathbf{QCoh}^{\mathcal{T}}(G(X))}(\mathbb{L}^{\mathcal{T}}_{G(X)},G(f)_{*}\phi(Y)(\pi_{n+1}(\mathcal{O}_{Y})[n+2]))&\cong\mathbf{Map}_{\mathbf{QCoh}^{\mathcal{T}}(G(X))}(\mathbb{L}^{\mathcal{T}}_{G(X)},\phi(X)f_{*}(\pi_{n+1}(\mathcal{O}_{Y})[n+2]))
\end{align*}
%\begin{align*}
%\mathbf{Map}(\Gamma^{\mathcal{T}}(X),\Gamma^{\mathcal{T}}(t_{\le n+1}(Y)))_{[f]}&\rightarrow \mathbf{Map}(\Gamma^{\mathcal{T}}(X),\Gamma^{\mathcal{T}}(t_{\le n}(Y)))_{[f]}\\
%&\rightarrow\mathbf{Map}_{{}_{\Gamma^{\mathcal{T}}(X})}\mathbf{Mod}^{\mathcal{T}}(\mathbb{L}^{\mathcal{T}}_{\Gamma^{\mathcal{T}}(X,\mathcal{O}_{X})},\Gamma^{\mathcal{T}}(Y,\pi_{n+1}(\mathcal{O}_{Y}))[n+1])
%\end{align*}
Using the inductive step and comparing fibre sequences gives the result.

% $$\mathbf{Map}(t_{\le n+1}Y,X)_{[f]}\rightarrow\mathbf{Map}(t_{\le n}Y,X)_{[f]}\rightarrow\mathbf{Map}_{\mathbf{Mod}^{\mathcal{T}}(X)}(f^{*}\mathbb{L}^{\mathcal{U}}_{X},\pi_{n+1}\mathcal{O}_{Y}[n+1])$$
%Since $\psi(Y):\mathbf{Mod}^{\mathcal{U}}(Y)\rightarrow\mathbf{Mod}^{\mathcal{T}}(G(Y))$ is exact, and both $Y$ and $G(Y)$ have constructibly convergent Postnikov towers, we have $\psi(t_{\le n}Y)\cong t_{\le n}\psi(Y)$. Thus we may assume that $t_{\le n}Y\rightarrow Y$ is an equivalence for some $n$, and the proof again proceeds by induction. The case $n=0$ is by assumption. Suppose we have proven the claim for some $n$. Let $f\in\pi_{0}(\mathbf{Map}(Y,X))$ we have a fibre sequence
%$$\mathbf{Map}(t_{\le n+1}Y,X)_{[f]}\rightarrow\mathbf{Map}(t_{\le n}Y,X)_{[f]}\rightarrow\mathbf{Map}_{\mathbf{Mod}^{\mathcal{T}}(X)}(f^{*}\mathbb{L}^{\mathcal{U}}_{X},\pi_{n+1}\mathcal{O}_{Y}[n+1])$$
%We also have a fibre sequence
%$$\mathbf{Map}(G(t_{\le n+1}Y),G(X))_{[G(f)]}\rightarrow\mathbf{Map}(G(t_{\le n}Y),G(X))_{[G(f)]}\rightarrow\mathbf{Map}_{\mathbf{Mod}^{\mathcal{U}}(G(X))}(G(f)^{*}\mathbb{L}^{\mathcal{T}}_{G(X)},\pi_{n+1}(\mathcal{O}_{G(Y)})[n+1])$$
 \end{proof}
 



%Since $G$ commutes with colimits we may assume that $t_{\le n}Y\rightarrow Y$ is an equivalence for some $n$. The proof is by induction of the Postnikov tower of $Y$.  When $Y\cong t_{\le0}(Y)$ then the claim is the first assumption.
%
%Now  we have a pullback diagram
%\begin{displaymath}
%\xymatrix{
%\mathbf{Map}(t_{\le n+1}Y,X)\ar[d]\ar[r] & \mathbf{Map}(t_{\le n}Y,X)\ar[d]\\
%\mathbf{Map}(t_{\le n}Y,X)\ar[r] & \mathbf{Map}((t_{\le n}Y[\pi_{n+1}\mathcal{O}_{Y}[n+1]],X))
%}
%\end{displaymath}
%For each $[f]\in\pi_{0}\mathbf{Map}(Y,X)$ we get a fibre sequence
%$$\mathbf{Map}(t_{\le n+1}Y,X)_{[f]}\rightarrow\mathbf{Map}(t_{\le n}Y,X)_{[f]}\rightarrow \mathbf{Map}_{\mathbf{Mod}^{\mathcal{U}}(X)}(\mathbb{L}^{\mathcal{U}}_{X},f_{*}\pi_{n+1}\mathcal{O}_{Y}[n+1])$$
%By assumption we have 
%\begin{align*}
% \mathbf{Map}_{\mathbf{Mod}^{\mathcal{U}}(X)}(\mathbb{L}^{\mathcal{U}}_{X},f_{*}\pi_{n+1}\mathcal{O}_{Y}[n+1])&\cong  \mathbf{Map}_{\mathbf{Mod}^{\mathcal{U}}(X)}(\psi(X)(\mathbb{L}_{G(X)}^{\mathcal{T}}),f_{*}\pi_{n+1}\mathcal{O}_{Y}[n+1])\\
% &\cong \mathbf{Map}_{\mathbf{Mod}(G(X))}(\mathbb{L}^{\mathcal{T}}_{G(X)},\phi(X)\circ f_{*}\pi_{n+1}\mathcal{O}_{Y}[n+1])
%\end{align*}
%\begin{align*}
% \mathbf{Map}_{\mathbf{QCoh}^{\mathcal{U}}(X)}(\mathbb{L}^{\mathcal{U}}_{X},f_{*}\pi_{n+1}\mathcal{O}_{Y}[n+1])&\cong  \mathbf{Map}_{\mathbf{QCoh}^{\mathcal{U}}(X)}(\mathcal{O}_{X}\otimes^{\mathcal{U}}_{\Gamma^{\mathcal{T}}(X)}\phi^{*}(\mathbb{L}^{\mathcal{T}}_{\Gamma^{\mathcal{T}}(X)}),f_{*}\pi_{n+1}\mathcal{O}_{Y}[n+1])\\
% &\cong\mathbf{Map}_{{}_{\Gamma^{\mathcal{U}}(X)}\mathbf{Mod}^{\mathcal{U}}}(\phi^{*}(\mathbb{L}^{\mathcal{T}}_{\Gamma^{\mathcal{T}}(X)}),\Gamma^{\mathcal{U}}(Y,\pi_{n+1}(\mathcal{O}_{Y}))[n+1])\\
% &\cong \mathbf{Map}_{{}_{\Gamma^{\mathcal{T}}(X)}\mathbf{Mod}^{\mathcal{T}}}(\mathbb{L}^{\mathcal{T}}_{\Gamma^{\mathcal{T}}(X)},\Gamma^{\mathcal{T}}(Y,\pi_{n+1}(\mathcal{O}_{Y}))[n+1])
%\end{align*}


\section{Extended Example: Geometry Relative to Symmetric Monoidal Categories}

Let us give our first example of an algebro-geometric context. It is somewhat trivial in that $\mathrm{Spec}$ and $\mathcal{O}$ are anti-equivalences.

\begin{construction}
Let $\mathbf{C}$ be a presentably symmetric monoidal $(\infty,1)$-category, and set $\mathbf{Aff}\defeq\mathbf{Comm}(\mathbf{C})^{op}$. Define $\mathbf{Str}$ to be the functor which sends $R^{op}$ to ${}_{R\big\backslash}\mathbf{Comm}(\mathbf{C})$. $\mathcal{O}$ sends $R^{op}\rightarrow S^{op}$ to $S\rightarrow R$, and $\mathrm{Spec}$ sends $S\rightarrow R$ to $R^{op}\rightarrow S^{op}$. By abuse of notation we refer to this pre-$(\infty,1)$-algebro-geometric tuple as $\mathbf{Aff_{C}}$.
\end{construction}

Note by \cite{HA} Remark 7.3.4.16, we have
$$\mathbf{Mod}(R^{op})\cong{}_{R}\mathbf{Mod}(\mathbf{Sp(C)})$$

\begin{example}
\begin{enumerate}
\item
Let $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ be a spectral algebraic pre-context. Define $\mathbf{Str}$ to be the functor which sends $R$ to $\mathbf{Comm}(\mathbf{Mod}^{\le0})_{\big\slash R}$. $\mathcal{O}$ sends $R^{op}\rightarrow S^{op}$ to $S\rightarrow R$, and $\mathrm{Spec}$ sends $S\rightarrow R$ to $R^{op})\rightarrow S^{op}$. $\mathbf{Mod}:\mathbf{Aff}\rightarrow\mathbf{Cat}$ is equivalent to the assignment $R^{op}\mapsto{}_{R}\mathbf{Mod}$.
%There is an equivalence $\mathbf{QCoh}\cong\mathbf{Sp(\mathbf{Ab(Str_{\big\slash(S)})})}\circ\mathcal{O}$.
\item
There is a stable version of the first example in which ${}_{R}\mathbf{Mod}^{\le0}$ is replaced by ${}_{R}\mathbf{Mod}$. Again $\mathbf{Mod}:\mathbf{Aff}\rightarrow\mathbf{Cat}$ is equivalent to the assignment $R^{op}\mapsto{}_{R}\mathbf{Mod}$.
\item
Let $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ be a derived algebraic context. The first two examples can be repeated, replacing $\mathbf{Comm}$ by $\mathbf{DAlg}$. 
\end{enumerate}
\end{example}

We can incorporate condensed geometry in this setup also.

\begin{construction}
Let $\mathbf{R}$ be a geometric category of connective decorated rings  in a derived algebraic context $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ as in \cite{kelly2021analytic} Definition 10.10. An object of such a category is, essentially, a pair $(R,\mathbf{M}_{R})$, where $R\in\mathbf{DAlg}^{cn}(\mathbf{C})$ and $\mathbf{M}_{R}$ is a reflective subcategory of ${}_{R}\mathbf{Mod}(\mathbf{C})$. We define $\mathbf{Aff}\defeq\mathbf{R}^{op}$. Define $\mathbf{Str}$ to be the functor which sends $R$ to $\mathbf{R}_{\big\slash R}$. $\mathcal{O}$ sends $R^{op}\rightarrow S^{op}$ to $S\rightarrow R$, and $\mathrm{Spec}$ sends $S\rightarrow R$ to $R^{op}\rightarrow S^{op}$ .Define
$$\mathbf{Mod}(R)\defeq\mathbf{M}_{R}$$
The square-zero extension functor is defined as in \cite{kelly2021analytic} Section 10. The contangent complex of any morphism in $\mathbf{Aff}$ exists, as shown in \cite{kelly2021analytic}. 
 \end{construction}
 
 \subsection{Geometry Relative to a Spectral Context}


Let us specialise to spectral contexts. In this situation it is natural to consider both connective and non-connective geometry.


%\begin{enumerate}
%\item
%a relative $(\infty,1)$ algebro-geometric context
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{QCoh},R)$$
%\item
%A full subcategory $\mathbf{A}\subset\mathbf{Aff}$ be a full subcategory stable by equivalences. 
%\item
%For each 
%\end{enumerate}



%\begin{defn}
%Let $(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0})$ be a spectral algebraic pre-context, $\tau$ a topology on $\mathbf{Aff}^{cn}_{\mathbf{C}}$ and $B\in\mathrm{CAlg}^{cn}(\mathbf{C})$. A $B$-module $M$ is said to \textit{satisfy  weak \v{C}ech descent} if for any cover $\{\mathrm{Spec}(A_{i})\rightarrow\mathrm{Spec}(A)\}_{i\in\mathcal{I}}$ in $\tau$ the natural map from $M$ to the homotopy limit of the cosimplicial diagram
%$$n\mapsto\prod_{(i_{0},\ldots,i_{n})\in\mathcal{I}^{n+1}}M\otimes_{A}A_{i_{0}}\otimes_{A}A_{i_{1}}\otimes_{A}\ldots\otimes_{A}A_{i_{n}}$$
%is an equivalence. $\tau$ is said to \textit{satisfy weak \v{C}ech descent} if for any $B\in\mathbf{DAlg}^{cn}(\mathbf{C})$, any $B$-module satisfies weak \v{C}ech descent.
%\end{defn}

%Let $f:A\rightarrow B$ be a map of commutative monoids, $M$ a stable $B$-module, and $d\in\pi_{0}(\mathrm{Der}_{A}(B,M))$. This defines a map of commutative monoids $d:B\rightarrow B\oplus M$. There is also the zero section map $s:B\rightarrow B\oplus M$. We consider the homotopy pullback
%\begin{displaymath}
%\xymatrix{
%C\ar[d]\ar[r] & B\ar[d]^{d}\\
%B\ar[r]^{s} & B\oplus M
%}
%\end{displaymath}
%As explained in \cite{toen2008homotopical} Section 1.2.1. The homotopy fibre of the map $C\rightarrow B$ is equivalent to the loops module $\Omega M$, so that $C$ is a square-zero extension of $B$ by $\Omega M$, which we denote by $B\oplus_{d}\Omega M$. Here $\Omega M$ is the \textit{loop module} of $M$ given by the pullback $0\times_{M}0$. 




%For integers $n$, we shall write
%$$\mathbf{F}_{A}^{n}\defeq\mathbf{F}_{A}\times_{\mathbf{Mod}_{A}}\mathbf{Mod}^{n}_{A}$$
%and in particular, $\mathbf{F}_{A}^{cn}\defeq\mathbf{F}_{A}^{0}$.

\begin{defn}

A \textit{weak relative \'{e}tale SAG context} is a tuple $(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0},\mathbf{D},\mathbf{\theta},\tau,\mathbf{P},\mathbf{A},\mathbf{F})$ where
\begin{enumerate}
\item
$(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0},\mathbf{D},\mathbf{\theta})$ is a spectral algebraic pre-context;
\item
$\tau$ is a Grothendieck topology on $\mathbf{Aff}_{\mathbf{D}}$;
\item
$\mathbf{P}$ is a class of maps in $\mathsf{Ho}(\mathbf{Aff}_{\mathbf{D}})$ which is stable by composition, pullback, and contains isomorphisms;
\item
$\mathbf{P}$ consists of formally \'{e}tale morphisms;
\item
$\mathbf{F}$ is a good system of modules on $\mathbf{A}$,
%\item
%$\tau^{qc}$ satisfies weak \v{C}ech descent.
%\item
%If $\mathrm{Spec}(A)$ in $\mathbf{A}$ then $\mathsf{L}\Omega^{1}_{A}\in\mathbf{Mod}^{\tau}_{A}$.
%\item
%$\tau$ satisfies weak \v{C}ech descent relative to $\mathbf{A}$ and $\mathbf{F}$.
\end{enumerate}
such that $(\mathbf{Aff}_{\mathbf{D}},\tau,\mathbf{P},\mathbf{A})$ is a strong relative $(\infty,1)$-geometry tuple. 
\end{defn}

\begin{defn}

A \textit{connective weak relative \'{e}tale SAG context} is a tuple $(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0},\mathbf{D},\mathbf{\theta},\tau,\mathbf{P},\mathbf{A},\mathbf{F})$ where
\begin{enumerate}
\item
$(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0},\mathbf{D},\mathbf{\theta})$ is a spectral algebraic pre-context;
\item
$\tau$ is a Grothendieck topology on $\mathbf{Aff}^{cn}_{\mathbf{D}}$;
\item
$\mathbf{P}$ is a class of maps in $\mathsf{Ho}(\mathbf{Aff}^{cn}_{\mathbf{D}})$ which is stable by composition, pullback, and contains isomorphisms;
\item
$\mathbf{P}$ consists of formally \'{e}tale morphisms;
\item
$\mathbf{F}$ is a good system of modules on $\mathbf{A}$,
%\item
%$\tau^{qc}$ satisfies weak \v{C}ech descent.
%\item
%If $\mathrm{Spec}(A)$ in $\mathbf{A}$ then $\mathsf{L}\Omega^{1}_{A}\in\mathbf{Mod}^{\tau}_{A}$.
%\item
%$\tau$ satisfies weak \v{C}ech descent relative to $\mathbf{A}$ and $\mathbf{F}$.
\end{enumerate}
such that $(\mathbf{Aff}^{cn}_{\mathbf{D}},\tau,\mathbf{P},\mathbf{A})$ is a strong relative $(\infty,1)$-geometry tuple. 
\end{defn}

\subsubsection{Higher (Underived) Geometry}

Let  $(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0},\mathbf{D},\mathbf{\theta},\tau,\mathbf{P},\mathbf{A},\mathbf{F})$ be a (connective) weak relative smooth SAG context. Let $\mathbf{A}^{\heart}$ denote the full subcategory of $\mathbf{Aff_{C}}^{cn}$ consisting of objects of the form $\mathrm{Spec}(A)$ where $\mathrm{Spec}(A)\in\mathbf{A}$, and $A\in\mathbf{C}^{\heart}$.

\begin{defn}
$(\mathbf{C},\mathbf{C}_{\ge0},\mathbf{C}_{\le0},\mathbf{C}^{0},\mathbf{D},\mathbf{\theta},\tau,\mathbf{P},\mathbf{A},\mathbf{F})$ is said to be a \textit{classical enhancement of }$\mathbf{A}^{\heart}$ if
\begin{enumerate}
\item
$(\mathbf{A},\tau|_{\mathbf{A}},\mathbf{P}|_{\mathbf{A},}\mathbf{A}^{\heart})$ is a strong relative $(\infty,1)$-geometry tuple. 
\item
for any $\mathrm{Spec}(A)\in\mathbf{A}$, $\pi_{0}(A)\in\mathbf{A}^{\heart}$
\end{enumerate}
\end{defn}
Then we get a fully faithful functor
$$\mathbf{Stk}(\mathbf{A}^{\heart},\tau|_{\mathbf{A}^{\heart}})\rightarrow\mathbf{Stk}(\mathbf{A},\tau|_{\mathbf{A}})$$
which induces a fully faithful functor between $n$-geometric stacks. $\mathbf{Stk}(\mathbf{A}^{\heart},\tau|_{\mathbf{A}^{\heart}})$ is the category of \textit{higher stacks} on the $1$-categorical Grothendieck site $(\mathbf{A}^{\heart},\tau|_{\mathbf{A}^{\heart}})$. The full subcategory of $\mathbf{Stk}(\mathbf{A}^{\heart},\tau|_{\mathbf{A}^{\heart}})$ consisting of $1$-truncated objects (i.e. sheaves of $1$-types) will be denoted $\mathrm{Stk}(\mathbf{A}^{\heart},\tau|_{\mathbf{A}^{\heart}})$. This is the `classical' category of stacks on  $(\mathbf{A}^{\heart},\tau|_{\mathbf{A}^{\heart}})$. 



\subsubsection{Strong Sites}

Often we will have the following set up. We fix a full subcategory $\mathbf{S}\subset\mathbf{Alg_{D}}(\mathbf{C}^{\heart})$, a class of maps $\mathbf{P}$ in $\mathbf{Alg}_{\mathbf{D}}(\mathbf{\mathbf{C}})$ stable by composition and pullbacks, and containing isomorphisms such that whenever $f:A\rightarrow B$ is a map in $\mathbf{P}|_{\mathbf{S}}$ and $A\rightarrow C$ is any map in $\mathbf{S}$, then $B\otimes_{A}^{\mathbb{L}}C\cong B\otimes_{A}C$ is an object of $\mathbf{S}$. For each $A\in\mathbf{S}$ we further fix a subcategory $\mathrm{M}_{A}\subset{}_{A}\Mod^{\heart}$ containing $A$, such that whenever $f:A\rightarrow B$ is a map in $\mathbf{P}|_{\mathbf{A}}$, and $N\in\mathrm{M}_{A}$, then $B\otimes_{A}^{\mathbb{L}}N\in\mathrm{M}_{B}$. 

\begin{defn}
\begin{enumerate}
\item
Let $\mathbf{dS}^{\mathrm{M}}$ denote the full subcategory of $\mathbf{DAlg}(\mathbf{C})^{cn}$ consisting of algebras $A$ such that 
\begin{enumerate}
\item
$\pi_{0}(A)\in\mathbf{S}$
\item
Each $\pi_{n}(A)\in\mathrm{M}_{\pi_{0}(A)}$.
\end{enumerate}
\item
Let $\mathbf{P}_{\mathbf{dS}}$ denote the set of maps $f:A\rightarrow B$ in $\mathbf{dS}^{\mathrm{M}}$ such that 
\begin{enumerate}
\item
$f$ is derived strong.
\item
$\pi_{0}(A)\rightarrow\pi_{0}(B)$ is in $\mathbf{P}|_{\mathbf{A}}$.
\end{enumerate}
\end{enumerate}
Further denote by $\mathbf{dS}^{\mathrm{M}}_{\le0}\subset \mathbf{dS}^{\mathrm{M}}$ the full subcategory consisting of objects $A$ such that $\pi_{i}(A)=0$ for $i>0$. 
\end{defn}

\begin{prop}\label{prop:cohtransv}
Let $\mathbf{S}$ and $\mathbf{P}$ be as above. Let $C\in\mathbf{S}$, and let $M\in\Mod(C)^{\heart}$ be such that for any $C\rightarrow D$ in $\mathbf{P}_{\mathbf{S}}$ the map
$$D\otimes_{C}^{\mathbb{L}}M\rightarrow D\otimes_{C}M$$
is an equivalence. Let $f:A\rightarrow B$ be a map in $\mathbf{P}_{\mathbf{S}}$, and $g:A\rightarrow C$ any map. Then $M$ is transverse to $B$ over $A$.
\end{prop}

\begin{proof}
The map $C\rightarrow B\otimes_{A}C\cong B\otimes_{A}^{\mathbb{L}}C$ is in $\mathbf{P}_{\mathbf{S}}$. Thus we have
\begin{align*}
B\otimes_{A}M&\cong (B\otimes_{A}C)\otimes_{C}M\\
&\cong (B\otimes_{A}C)\otimes^{\mathbb{L}}_{C}M\\
&\cong (B\otimes_{A}^{\mathbb{L}}C)\otimes^{\mathbb{L}}_{C}M\\
&\cong B\otimes_{A}^{\mathbb{L}}M
\end{align*}
as required.
\end{proof}

\begin{lem}
\begin{enumerate}
\item
The class $\mathbf{P}_{\mathbf{dS}}$ is closed under composition and contains equivalences. 
\item
If $A\rightarrow B$ is a map in $\mathbf{P}_{\mathbf{dS}}$ between objects in $\mathbf{dS}^{\mathrm{M}}$, and $A\rightarrow C$ is any map in $\mathbf{dS}^{\mathrm{M}}$, then $B\otimes_{A}^{\mathbb{L}}C\in\mathbf{dS}^{\mathrm{M}}$, and the map
$$C\rightarrow B\otimes_{A}^{\mathbb{L}}C$$
is in $\mathbf{P}_{\mathbf{dS}}$. Moreover if $C\in\mathbf{S}$ (resp. $C\in\mathbf{dS}^{\mathrm{M}}_{\le0}$)
\end{enumerate}
\end{lem}

\begin{proof}
The first part is clear, so we prove the second. By virtue of Proposition \ref{prop:cohtransv} we may use Proposition \ref{prop:derstronghtpy}. We get
$$\pi_{*}(B\otimes^{\mathbb{L}}_{A}C)\cong\pi_{0}(B)\otimes_{\pi_{0}(A)}\pi_{*}(C)$$
Thus 
$$\pi_{0}(B\otimes^{\mathbb{L}}_{A}C)\cong \pi_{0}(B)\otimes^{\mathbb{L}}_{\pi_{0}(A)}\pi_{*}(C)$$
is in $\mathbf{S}$ by assumption. Moreover, we have
$$\pi_{*}(B\otimes^{\mathbb{L}}_{A}C)\cong\pi_{0}(B)\otimes^{\mathbb{L}}_{\pi_{0}(A)}\pi_{*}(C)$$
Clearly then $\pi_{0}(B\otimes^{\mathbb{L}}_{A}C)\in\mathbf{S}$ and each $\pi_{n}(M)\in\mathrm{M}_{\pi_{0}(B\otimes^{\mathbb{L}}_{A}C)}$. 

Note in particular that if $C\in\mathbf{S}$ (resp. $\mathbf{dS}^{\mathrm{M}}_{\le0}$) then so is $B\otimes^{\mathbb{L}}_{A}C$. 
\end{proof}

\textcolor{red}{fix: fill out this subsection}


Rhiannon Savage is working on a vast generalisation of the representability theorem of \cite{toen2008homotopical} which will show that a stack $\mathcal{X}\in\mathbf{Stk}(\mathbf{A},\tau|_{\mathbf{A}})$ is $n$-geometric precisely if the classical truncation $t_{0}(\mathcal{X})$ is $n$-geometric and $\mathcal{X}$ has an obstruction theory. 



\section{Extended Example: Structured Spaces}

In this section we apply the formalism to a somewhat less trivial example, namely categories of structured spaces. 

\subsection{Pregeometries}

\begin{defn}[\cite{DAG V} 3.1.1]
A \textit{pregeometry} is an $\infty$-category $\mathcal{T}$, equipped with a class $\mathbf{P}$ of \textit{admissible morphisms}, and a Grothendieck topology $\tau$ such that
\begin{enumerate}
\item
$\mathcal{T}$ admits finite products.
\item
The pullback of a map in $\mathbf{P}$ along any morphisms exists.
\item
$\mathbf{P}$ is closed under composition, pullback, and retract, and if $f,g$ are morphisms such that $g$ and $g\circ f$ in $\mathbf{P}$, then $f\in\mathbf{P}$.
\item
If $\{X_{i}\rightarrow X\}$ is a cover in $\tau$ then each $X_{i}\rightarrow X$ is in $\mathbf{P}$.
\end{enumerate}
\end{defn}

\begin{defn}[\cite{DAG V} 3.1.4]
Let $\mathcal{T}$ be a pregeometry and let $\mathcal{X}$ be an $\infty$-topos. A $\mathcal{T}$-\textit{structure} on $\mathcal{X}$ is a functor $\mathcal{O}:\mathcal{T}\rightarrow\mathcal{X}$ such that
\begin{enumerate}
\item
The functor $\mathcal{O}$ preserves finite products.
\item
Given a pullback diagram
\begin{displaymath}
\xymatrix{
U'\ar[d]\ar[r] & U\ar[d]^{f}\\
X'\ar[r] & X
}
\end{displaymath}
in $\mathcal{T}$ where $f\in\mathbf{P}$, then 
\begin{displaymath}
\xymatrix{
\mathcal{O}(U')\ar[d]\ar[r] & \mathcal{O}(U)\ar[d]^{f}\\
\mathcal{O}(X')\ar[r] & \mathcal{O}_{X}
}
\end{displaymath}
is a pullback square in $\mathcal{X}$.
\item
Let $\{U_{\alpha}\rightarrow X\}$ be a covering in $\mathcal{T}$. Then the induced map
$$\coprod_{\alpha}\mathcal{O}(U_{\alpha})\rightarrow\mathcal{O}_{X}$$
is an effective epimorphism in $\mathcal{X}$.
\end{enumerate}
\end{defn}




\begin{defn}[\cite{DAG V}]
A \textit{morphism of }$\mathcal{T}$-\textit{structures} is just a natural transformation of functors $\mathcal{O}\rightarrow\mathcal{O}'$. A morphism is said to be \textit{local} if for every admissible $U\rightarrow X$ in $\mathcal{T}$ the diagram
\begin{displaymath}
\xymatrix{
\mathcal{O}(U)\ar[d]\ar[r] & \mathcal{O}'(U)\ar[d]\\
\mathcal{O}_{X}\ar[r] & \mathcal{O}'(X)
}
\end{displaymath}
is a pullback square. Denote by $\mathbf{Str}_{\mathcal{T}}^{loc}(\mathcal{X})$ the category of $\mathcal{T}$-structures on $\mathcal{X}$ with local morphisms.
\end{defn}

\begin{construction}
Let $\mathcal{T}$ be a pregeometry. Define $\mathbf{Aff}\defeq{}^{L}\mathbf{Top}(\mathcal{T})$ to be the category of $\mathcal{T}$-structured spaces. $\mathbf{Str}$ sends $(\mathcal{X},\mathcal{O}_{X})$ to ${}_{\mathcal{O}_{X}\big\backslash}\mathbf{Str}^{loc}_{\mathcal{T}}(\mathcal{X})$. $\mathcal{O}$ sends $(f,f^{\#}):(Y,\mathcal{O}_{Y})\rightarrow(X,\mathcal{O}_{X})$ to $\mathcal{O}_{X}\rightarrow f_{*}\mathcal{O}_{Y}$. $\mathrm{Spec}$ sends $\tilde{\mathcal{O}}_{X}\in{}_{\mathcal{O}_{X}\big\backslash}\mathbf{Str}^{loc}_{\mathcal{T}}(\mathcal{X})$ to the natural map $(\mathcal{X},\tilde{\mathcal{O}}_{X})\rightarrow (\mathcal{X},\mathcal{O}_{X})$. We will return to this class of examples later. 
We shall denote the pre-$(\infty,1)$-algebro-geometric tuple associated to a pre-geometry $\mathcal{T}$ by 
$$\mathbf{StrSp}(\mathcal{T})$$
\end{construction}

Let us give an important example.

\begin{example}[\cite{DAG V} Example 3.1.3]
Let $\mathcal{T}$ be any small $\infty$-category which admits finite products. The \textit{trivial pregeometry} structure on $\mathcal{T}$ has the class of equivalences as $\mathbf{P}$, and any non-empty collection of equivalences as covers in $\tau$. We denote this pregeometry by $\mathcal{T}^{disc}$. Note that in this case $\mathbf{Str}^{loc}(\mathcal{X})$ is just the category of finite product preserving functors from $\mathcal{T}$ to $\mathcal{X}$,
$$\mathbf{Fun}^{\times}(\mathcal{T},\mathcal{X})$$
For $\mathcal{X}=\mathbf{sSet}$, this is precisely the free sifted cocompletion of $\mathbf{P}_{\Sigma}(\mathcal{T}^{op})$. For general $\mathcal{X}$, an object of $\mathbf{Str}^{loc}(\mathcal{X})$ is a $$\mathbf{P}_{\Sigma}(\mathcal{T}^{op})$$-valued sheaf on $\mathcal{X}$ by \cite{DAGV} Example 3.1.6. 
%Let $\mathcal{T}$ be a small $\infty$-category which admits finite products. Let $\mathrm{Rec}(\mathcal{T}^{op})$ denote the free cocompletion of $\mathcal{T}^{op}$ under geometric realisations. Equip this category $(\mathrm{Rec}(\mathcal{T}^{op}))^{op}$ with the trivial pregeometry structure. Then $\mathbf{Str}_{\mathrm{Rec}(\mathcal{T}^{op})}^{loc}(\mathcal{X})$ is the category of $\mathbf{P}_{\Sigma}(\mathcal{T}^{op})$-valued sheaves on $\mathcal{X}$, where $\mathbf{P}_{\Sigma}(\mathcal{T}^{op})$ is the free sifted cocompletion of $\mathcal{T}^{op}$. We write $\mathcal{T}^{\Sigma,disc}\defeq((\mathrm{Rec}(\mathcal{T}^{op}))^{op})^{disc}$
\end{example}


\subsection{Comparing Pregeometries}

\begin{defn}[\cite{lurie2009derived} Definition 3.2.1]
Let $\mathcal{T}$ and $\mathcal{U}$ be pregeometries. A \textit{transformation of pregeometries from} $\mathcal{T}$ \textit{to} $\mathcal{U}$ is a functor $\theta:\mathcal{T}\rightarrow\mathcal{U}$ such that
\begin{enumerate}
\item
$\theta$ preserves finite limits. 
\item
$\theta$ sends admissible morphisms in $\mathcal{T}$ to admissible morphisms in $\mathcal{U}$.
\item
$\theta$ sends covers in $\mathcal{T}$ to covers in $\mathcal{U}$.
\item
$\theta$ preserves pullbacks along admissible morphisms.
\end{enumerate}
\end{defn}

\begin{defn}[\cite{lurie2009derived}]
A transformation of pre-geometries $\phi:\mathcal{T}\rightarrow\mathcal{U}$ is said to be a \textit{Morita equivalence} if for any $\infty$-topos $\mathcal{X}$ the adjunction
 $$\phi_{*}:\mathbf{Str}_{\mathcal{U}}^{loc}(\mathcal{X})\rightarrow\mathbf{Str}_{\mathcal{T}}^{loc}(\mathcal{X})$$
 is an equivalence. 
\end{defn}


The following is essentially a part of \cite{lurie2009derived} Proposition 3.2.8.

\begin{lem}
Let $\phi:\mathcal{T}\rightarrow\mathcal{U}$ be a transformation of pregeometries. Suppose that
\begin{enumerate}
\item
$\phi$ is fully faithful.
%\item
%If $f:S\rightarrow T$ is admissible in $\mathcal{T}$ if and only if $\phi(f)$ is admissible in $\mathcal{U}$.
%\item
%A collection of maps $\{T_{i}\rightarrow T\}$ is a cover in $\mathcal{T}$ if and only if $\{\phi(T_{i})\rightarrow \phi(T)\}$ is a cover in $\mathcal{U}$.
\item
For any object $U$ of $\mathcal{U}$ there exists a cover $\{\phi(T_{i})\rightarrow U\}$ in $\mathcal{U}$ where each $T_{i}\in\mathcal{T}$. 
\item
For any pullback diagram
\begin{displaymath}
\xymatrix{
U\times_{X}V\ar[d]\ar[r] & U\ar[d]^{f}\\
V\ar[r]^{g} & X
}
\end{displaymath}
in $\mathcal{T}$ where $f$ and $g$ are admissible and $U,V$ are in $\mathcal{T}$, then $U\times_{X}V$ is in $\mathcal{T}$. 
\end{enumerate}
The the functor
$$\phi_{*}:\mathbf{Str}_{\mathcal{U}}(\mathcal{X})\rightarrow\mathbf{Str}_{\mathcal{T}}(\mathcal{X})$$
is faithful and conservative.
\end{lem}

\begin{proof}
Let $f,g\in\pi_{0}\mathbf{Map}_{\mathbf{Str}^{loc}_{\mathcal{U}}(\mathcal{X})}\mathcal{O}\rightarrow\mathcal{O}'$ be such that $\phi_{*}(f)=\phi_{*}(g)$. Let $U\in\mathcal{U}$ and let $\{\phi(T_{i})\rightarrow U\}_{i\in\mathcal{I}}$ in $\mathcal{U}$ where each $T_{i}\in\mathcal{T}$. Then $f(T_{i})=f(U)$. Now 
$$\mathcal{O}(U)\cong\mathrm{colim}_{n,(i_{1},\ldots,i_{n})\in\mathcal{I}^{n}}\mathcal{O}(\phi(T_{i_{1}}))\times_{\mathcal{O}(U)}\times\ldots\times_{\mathcal{O}(U)}\mathcal{O}(\phi(T_{i_{1}}))\cong\mathrm{colim}_{n,(i_{1},\ldots,i_{n})\in\mathcal{I}^{n}}\mathcal{O}(\phi(T_{i_{1}}\times_{U}\times\ldots\times_{U}T_{i_{1}}))$$
Similarly 
$$\mathcal{O}'(U)\cong\mathrm{colim}_{n,(i_{1},\ldots,i_{n})\in\mathcal{I}^{n}}\mathcal{O}'(\phi(T_{i_{1}}\times_{U}\times\ldots\times_{U}T_{i_{1}}))$$
The claim now follows immediately, and the claim that $\phi_{*}$ reflects equivalences is similar. 
\end{proof}

A transformation of pregeometries $\theta:\mathcal{T}\rightarrow\mathcal{U}$ determines a map of pre-geometric tuples as follows. We get a functor 
$$G_{\theta}:{}^{L}\mathbf{Top}(\mathcal{U})\rightarrow{}^{L}\mathbf{Top}(\mathcal{T})$$
given by composition with $\theta$. In the same way we get an obvious natural transformation 
$$\phi_{\theta}:\mathbf{Str}_{\mathcal{U}}\rightarrow\mathbf{Str}_{\mathcal{T}}\circ G_{\theta}$$
also given by composition with $\theta$. It is straightforward to check that this determines a morphism of pre-geometric tuples. 

We also define
$$\Gamma^{\theta}:\defeq\Gamma^{\mathcal{T}}\circ G_{\theta}$$
When $\mathcal{T}\subset\mathcal{U}$ is a full subcategory and $\theta:\mathcal{T}\rightarrow\mathcal{U}$ is the inclusion, we write 
$$\Gamma^{\mathcal{T}}\defeq\Gamma^{\theta}$$



\subsubsection{Derived Algebraic Contexts and Pregeometries}

Let $\mathrm{C}$ be a monoidal elementary abelian category, so that 
$$\mathbf{DAlg}^{cn}(\mathrm{C})\cong\mathbf{P}_{\Sigma}(N(\mathrm{Sym}(P):P\in\mathcal{P}))$$
where $\mathcal{P}$ is a set of compact projective generators of $\mathrm{C}$ containing $\{k^{\oplus n}:n\in\mathbb{N}_{0}\}$, where $k$ is the monoidal unit. We define $\mathcal{T}^{\mathrm{Sym}(\mathcal{P})}$ to be the trivial pregeometry on the category $\{\mathrm{Sym}(P):P\in\mathcal{P}\}$. In this case we have 
$$\mathbf{Str}^{loc}_{\mathcal{T}^{\mathrm{Sym}(\mathcal{P})}}(\mathbf{sSet})\cong \mathbf{DAlg}^{cn}(\mathrm{C})$$
For $A\in\mathbf{DAlg}^{cn}(\mathrm{C})$ we have 
$${}_{A}\mathbf{Mod}^{\mathcal{T}^{\mathrm{Sym}(\mathcal{P})}}\cong {}_{A}\mathbf{Mod}(\mathbf{C})$$
If $A\rightarrow B$ is a map in $\mathbf{DAlg}^{cn}(\mathrm{C})$ then $$\mathbb{L}^{\mathcal{T}^{\mathrm{Sym}(\mathcal{P})}}_{A\big\slash B}\cong\mathbb{L}_{A\big\slash B}$$

%\begin{defn}
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$$
%is said to be $\mathrm{C}$-\textit{Fermat} if there is a morphism
%$(G,\phi,\delta,\epsilon)$of pre-$(\infty,1)$-algebro-geometric tuples
%to
%$$\mathbf{StrSp}(\mathcal{T}^{\mathcal{T}^{\mathrm{Sym}(\mathcal{P})}})$$
%such that for any $X\in\mathbf{Aff}$ the functor
%$$\mathbf{QCoh}(X)\rightarrow{}_{\mathcal{O}_{(G(X))}}\mathbf{Mod}$$
%is an equivalence of categories.
%\end{defn}
%$\mathcal{T}$ is said to be a $\mathbf{C}$-\textit{Fermat pre-geometry} if for any $A\in\mathbf{Str}^{loc}_{\mathcal{T}}(\mathbf{sSet})$  the functor
%$${}_{A}\mathbf{Mod}(\mathbf{C})\rightarrow\mathbf{Sp(Ab(Str}^{loc}_{\mathcal{T}}(\mathcal{X})\mathbf{))}$$
%is an equivalence of stable $\infty$-categories. 

 
%Let $(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ and $(\mathbf{D},\mathbf{D}^{\le0},\mathbf{D}^{\ge0},\mathbf{D}^{0})$ be a derived algebraic contexts, and let 
%$$F:\mathbf{D}^{0}\subset\mathbf{C}^{0}$$
%be a strictly symmetric monoidal functor. Then we have a functor
%$$\mathrm{Sym}(\mathbf{D}^{0})\rightarrow\mathrm{Sym}(\mathbf{C}^{0})$$
%and hence a map of pregeometries
%$$\phi:\mathcal{T}^{\mathrm{Sym}(\mathbf{D}^{0})}\rightarrow\mathcal{T}^{\mathrm{Sym}(\mathbf{C}^{0})}$$
%
%For any $\infty$-topos $\mathcal{X}$ we get an adjunction
%$$\adj{\phi^{*}}{\mathbf{Str}^{loc}_{\mathcal{T}^{\mathrm{Sym}(\mathbf{C}^{0})}}(\mathcal{X})}{\mathbf{Str}^{loc}_{\mathcal{T}^{\mathrm{Sym}(\mathbf{D}^{0})}}(\mathcal{X})}{\phi^{*}}$$
% In particular for $A\rightarrow B\in\mathbf{DAlg}^{cn}(\mathbf{C})$ we have a map
%$$\mathbb{L}_{\phi^{*}(A)\big\slash\phi^{*}(B)}\rightarrow\phi^{*}(\mathbb{L}_{A\big\slash B})$$

\begin{example}
\textcolor{blue}{edit:put earlier}
Let $R\in\mathbf{C}^{0}$ be the unit of $\mathbf{C}$. Then there is a map of pregeometries a
$$i:\mathbb{A}_{\mathrm{Hom}_{\mathbf{C}^{0}}(R,R)}\rightarrow\mathcal{T}^{\mathrm{Sym}(\mathbf{C}^{0})}$$
We write
$$(-)_{alg}\defeq i_{*}$$
\end{example}

%Let $\mathcal{T}$ be a pre-geometry equipped with a morphism of pregeometries
%$$\phi:\mathcal{T}^{\mathrm{Sym}(\mathcal{P})}\rightarrow\mathcal{T}$$
%and let $A\in\mathbf{Str}^{loc}_{\mathcal{T}}(\mathbf{sSet})$. We get an adjunction
%$$\adj{\phi^{*}}{{}_{\phi_{*}(A)}\mathbf{Mod(C)}}{{}_{A}\mathbf{Mod}^{\mathcal{T}}}{\phi_{*}}$$

\subsubsection{Pregeometries and Lawvere Theories}

For $\mathrm{T}$ an $\underline{\Lambda}$-sorted Lawvere theory, let $\mathcal{T}^{\mathrm{T}}$ denote the pregeometry defined as follows. As an $\infty$-category it is the nerve $N(\mathrm{Alg_{T}^{ffg}})$. The pregeometry structure is the trivial one. In particular we have an equivalence
$$\mathbf{Str}^{loc}_{\mathcal{T}^{\mathrm{T}}}(\mathbf{sSet})\cong\mathbf{sAlg}_{\mathrm{T}}$$
Suppose that $\Lambda$ is a partially ordered abelian group, and that $\mathrm{T}$ is an $\underline{\Lambda}$-sorted Fermat theory. Then for any $A^{op}\in\mathbf{Aff}_{\mathcal{T}^{\mathrm{T}}}(\bullet)$ we have 
$$\mathbf{Mod}(A^{op})\cong{}_{A_{alg}^{\underline{\Lambda}}}\mathbf{Mod}$$
Moreover by comparing the definitinos, for $f^{op}:B^{op}\rightarrow A^{op}\in\mathbf{Aff}_{\mathcal{T}^{\mathrm{T}}}(\bullet)$, the contangent complex of $f^{op}$ exists, and coincides with the cotangent complex of $f:A\rightarrow B$ as a map of $\mathrm{T}$-algebras defined in \cite{subsec:lawerecotangent}.

%Now let $A\in\mathrm{sAlg_{T}}$. The truncation $\tau^{\ge-n}A$ has a natural $\mathrm{T}$-algebra structure. Consider the natural map of $\mathrm{T}$-algebras $\tau^{\ge-n}A\rightarrow \tau^{\ge-n+1}A$ and the homotopy pushout
%
%\begin{displaymath}
%\xymatrix{
%\tau^{\ge-n}A\ar[d]\ar[r] & \tau^{\ge-n+1}A\ar[d]\\
%\tau^{\ge-n+1}A\ar[r] & B
%}
%\end{displaymath}
%The identity of $ \tau^{\ge-n+1}A$ induces a map $B\rightarrow \tau^{\ge-n+1}A$ such that the composite $ \tau^{\ge-n+1}A\rightarrow B\rightarrow  \tau^{\ge-n+1}A$ is the identity. Consider the truncation of this diagram, which is also a homotopy pushout square.
%
%\begin{displaymath}
%\xymatrix{
%\tau^{\ge-n}A\ar[d]\ar[r] & \tau^{\ge-n+1}A\ar[d]^{s}\\
%\tau^{\ge-n+1}A\ar[r] & \tau^{\ge-n+1}B
%}
%\end{displaymath}
%$s$ has a retraction, and thus is isomorphic to the zero derivation $\tau^{\ge-n+1}A\rightarrow\tau^{\ge-n+1}A\oplus\Sigma_{-n+1}\pi_{n}(A)$. The top horizontal map is then a square-zero extension by a derivation $d_{n}$. Moreover the diagram
%\begin{displaymath}
%\xymatrix{
%\tau^{\ge-n}A\ar[d]\ar[r] & \tau^{\ge-n+1}A\ar[d]^{s}\\
%\tau^{\ge-n+1}A\ar[r] & \tau^{\ge-n+1}B
%}
%\end{displaymath}
%is a pullback diagram (since it is so after forgetting to underlying filtered rings). 
%
%Thus we have proven the following.
%
%\begin{lem}
%Every object 
%\end{lem}

\subsubsection{Fermat Theories}

Let $\underline{\mathbf{C}}=(\mathbf{C},\mathbf{C}^{\le0},\mathbf{C}^{\ge0},\mathbf{C}^{0})$ be a derived algebraic context.

\begin{defn}
A pregeometry $\mathcal{U}$ is said to be $\underline{\mathbf{C}}$-\textit{pre-Fermat} if there is a transformation of pre-geometries
$$\mathcal{T}^{\underline{\mathbf{C}}}\rightarrow\mathcal{U}$$
\end{defn}

If $\mathcal{U}$ is a $\underline{\mathbf{C}}$-pre-Fermat pregeometry, we get a forgetful functor

$$(-)_{\underline{\mathbf{C}}}^{alg}:\mathbf{Str}_{\mathcal{U}}^{loc}(\mathcal{X})\rightarrow\mathbf{Shv}(\mathcal{X},\mathbf{DAlg}^{cn}_{\underline{\mathbf{C}}})$$
 If $(\mathcal{X},\mathcal{O_{X}})\in{}^{L}\mathbf{Top}(\mathcal{U})$ there is an induced functor 
$$(-)^{alg}:{}_{\mathcal{O}_{X}}\mathbf{Mod}(\mathcal{X})\rightarrow{}_{(\mathcal{O}_{X})^{alg}_{\underline{\mathbf{C}}}}\mathbf{Mod}(\mathcal{X})$$

\begin{defn}
$\mathcal{U}$ is said to be \textit{weak} $\underline{\mathbf{C}}$-\textit{Fermat} if 
\begin{enumerate}
\item
For each $\infty$-topos $\mathcal{X}$ the functor
$$(-)_{\underline{\mathbf{C}}}^{alg}:\mathbf{Str}_{\mathcal{U}}^{loc}(\mathcal{X})\rightarrow\mathbf{Shv}(\mathcal{X},\mathbf{DAlg}^{cn}_{\underline{\mathbf{C}}})$$
is conservative.
\item
for each $(\mathcal{X},\mathcal{O_{X}})\in{}^{L}\mathbf{Top}(\mathcal{U})$ the functor 
$$(-)^{alg}:{}_{\mathcal{O}_{X}}\mathbf{Mod}(\mathcal{X})\rightarrow{}_{(\mathcal{O}_{X})^{alg}_{\underline{\mathbf{C}}}}\mathbf{Mod}(\mathcal{X})$$
is an conservative.
\end{enumerate}
\end{defn}

Exactly as in \cite{https://arxiv.org/pdf/1704.01683.pdf} Section 4.3.

\begin{lem}
A  $\underline{\mathbf{C}}$-pre-Fermat pregeometry $\mathcal{T}^{\underline{\mathbf{C}}}\rightarrow\mathcal{U}$ is $\underline{\mathbf{C}}$ if and only if for any $A\in\mathbf{Str}_{\mathcal{U}}^{loc}(\mathbf{sSet})$ the functor
$$(-)_{\underline{\mathbf{C}}}^{alg}:{}_{A}\mathbf{Mod}(\mathbf{sSet})\rightarrow{}_{(A)^{alg}_{\underline{\mathbf{C}}}}\mathbf{Mod}(\mathbf{sSet})$$
is an equivalence.
\end{lem}

From now on when the context is clear we will simply write $(-)^{alg}$ instead of $(-)_{\underline{\mathbf{C}}}^{alg}$.  

\begin{example}
Let $\underline{\Lambda}$ be a partially ordered abelian group and $\mathrm{T}$ a $\underline{\Lambda}$-filtered Fermat theory. Then $\mathcal{T}^{\mathrm{T}}$ is a $\underline{\mathrm{Filt_{\underline{\Lambda}}}}$-pre-Fermat pregeometry. 
\end{example}

\begin{defn}
A  $\underline{\mathbf{C}}$-pre-Fermat pregeometry $\mathcal{U}$ is said to be \textit{unramified} if the morphism of pregeometries
$$\mathcal{T}^{\underline{\mathbf{C}}}\rightarrow\mathcal{U}$$
is an unramified morphism of pregeometries in the sense of \cite{DAGIX} Definition 10.1.
\end{defn}

\begin{example}
Any morphism of discrete pregeometries is unramified. Thus any  $\underline{\mathbf{C}}$-pre-Fermat pregeometry which is discrete as a pregeometry is unramified. 
\end{example}

Exactly as in \cite{https://arxiv.org/pdf/1704.01683.pdf} Theorem 5.29 we have the following.

\begin{thm}
Let $\mathcal{U}$ be an unramified  $\underline{\mathbf{C}}$-pre-Fermat pregeometry, and let $\mathcal{A}\rightarrow \mathcal{B}$ be an effective epimorphism $\mathbf{Str}_{\mathcal{U}}^{loc}(\mathcal{X})$. Then the natural map
$$\mathbb{L}_{\mathcal{B}_{\underline{\mathbf{C}}}^{alg}\big\slash\mathcal{A}_{\underline{\mathbf{C}}}^{alg}}\rightarrow(\mathbb{L}_{\mathcal{B}\big\slash\mathcal{A}})_{\underline{\mathbf{C}}}^{alg}$$
is an equivalence.
\end{thm}

\begin{defn}
A  $\underline{\mathbf{C}}$-pre-Fermat pregeometry $\mathcal{U}$ is said to be \textit{compatible with truncations} if $\mathcal{U}$ is compatible with truncations as a pregeometry.
\end{defn}

\begin{lem}
Let $\mathcal{U}$ be an unramified $\underline{\mathbf{C}}$-Fermat pregeometry which is compatible with truncations. Then any $A\in\mathbf{Str}^{loc}_{\mathcal{U}}(\mathbf{sSet})$ has a constructibly convergent Postnikov tower.
\end{lem}

\begin{proof}
The forgetful functor $(-)^{alg}_{\underline{\mathbf{C}}}$ commutes with filtered colimits and is conservative. The proof now follows by  an identical method to \cite{https://arxiv.org/pdf/1704.01683.pdf} Corollary 5.44.
\end{proof}

%\subsubsection{Embedding Multi-sorted Lawvere Theories in Derived Algebraic Contexts}\label{subsec:embedmulti}
%
%Let $\underline{\Lambda}$ be a partially ordered abelian group, $\mathrm{T}$ a $\underline{\Lambda}$-sorted Fermat theory. Furthermore let $\mathrm{C}$ be a monoidal elementary abelian category and $F:\mathrm{T}^{op}\rightarrow\mathrm{Comm(C)}$ a functor realising $\mathrm{T}$ as a Lawvere theory of $\mathrm{C}$-polynomial type. This gives rise to a transformation of pregeometries
%$$\mathcal{T}^{\mathrm{T}}\rightarrow\mathcal{T}^{\mathbf{DAlg}^{cn}(\mathbf{Ch}(\mathrm{C}))}$$
%Let $\mathbf{Q}\subset\mathbf{sAlg}_{\mathrm{T}}$ be a full subcategory such that the functor
% $$\pi_{0}(\mathbf{Q})\rightarrow\mathrm{Comm}(\mathrm{C})$$ 
% is fully faithful, where $\pi_{0}(\mathbf{Q})\subset\mathrm{Alg_{T}}$ is the full subcategory consisting of algebras of the form $\pi_{0}(Q)$ where $Q\in\mathbf{Q}$. We claim that the functor
% $$\mathbf{Q}\rightarrow\mathbf{DAlg}^{cn}(\mathbf{Ch}(\mathrm{C})))$$
% is fully faithful. By the previous section any $Q\in\mathbf{Q}$ has a constructibly convergent Postnikov tower. Thus it suffices to prove that for $Q\in\mathbf{Q}$ the map
%$$F(\mathbb{L}_{Q})\rightarrow\mathbb{L}_{F(Q)}$$
%is an equivalence. Now $Q$ has a presentation 
%$$Q\cong\mathrm{Free_{T}}(X)$$
%where $X$ is a $\underline{\Lambda}$-filtered simplicial set. Then $\mathbb{L}_{\mathrm{Free_{T}}(X)}$ is the realisation of the simplicial object given in degree $n$ by $\coprod_{|X_{n}|}\mathrm{Free_{T}}(X_{n})$, where $|X_{n}|$ denotes the underlying set of the filtered set $X_{n}$. Since $F$ is colimit-preserving we have $F(\mathbb{L}_{Q})$ is the realisation of the simplicial diagram which in degree $n$ is $\coprod_{X_{n}}F(\mathrm{Free_{T}}(X_{n}))$. However since the map $S(|X|)\rightarrow F(\mathrm{Free_{T}}(X))$ is a homotopy epimorphism, this is equivalent to $\mathbb{L}_{F(Q)}$. 

%\subsubsection{Localisation}
%
%Let 
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{F})$$
%be a pre-$(\infty,1)$-algebro-geometric tuple. Consider the global sections morphism $\Gamma$. 
%\begin{defn}
%A full subcategory $\mathbf{A}\subset\mathbf{Aff}$ is said to be \textit{localisable} if
%\begin{enumerate}
%\item
%$\Gamma$ is fully faithful when restricted to $0$-truncated objects in $\mathbf{A}$.
%\item
%
%\item
%For $X\in\mathbf{A}$ the functor
%$$\Gamma:\mathbf{Mod}(X)\rightarrow\mathbf{Mod}(\Gamma(X))$$
%restricts to a fully faithul functor on $\mathbf{F}_{X}$. 
%\item
%Every object $X\in\mathbf{A}$ has a cotangent complex in $\mathbf{F}_{X}$, and a constructibly convergent Postnikov tower.
%\end{enumerate}
%\end{defn}
%
%Let  be a full subcategory such that $\Gamma$ is fully faithful when restricted to $0$-truncated objects. Suppose further that for any $X\in\mathbf{A}$ we have $\mathbb{L}_{X}\in\mathbf{F}_{X}$. We claim that the restriction of $\Gamma$ to $\mathbf{A}$ is fully faithful. For this it suffices to show that 
%
%We have
%
%\begin{align*}
%\mathbf{Map}(\mathcal{O}_{X}\otimes\mathbb{L}_{\Gamma(X)}),M)&\cong\mathbf{Map}(\mathbb{L}_{X},M)\\
%&\cong\mathbf{Map}_{X\big\backslash\mathbf{Aff}}(X[M],X)
%\end{align*}


\subsection{Comparison of (Pre-)Fermat Pre-geometries}

Let $\underline{\mathbf{C}}$ and $\underline{\mathbf{D}}$ be derived algebra contexts, and let $F:\underline{\mathbf{C}}\rightarrow\underline{\mathbf{D}}$ be a morphism of derived algebra contexts such that for any map $\mathcal{A}\rightarrow \mathcal{B}\in\mathbf{Shv}(\mathcal{X},\mathbf{DAlg}^{cn}(\mathbf{C}))$ the map $F(\mathbb{L}_{\mathcal{B}\big\slash\mathcal{A}})\rightarrow\mathbb{L}_{(F(\mathcal{B})\big\slash F(\mathcal{A}))}$ is an equivalence. Let $\mathcal{T}^{\underline{\mathbf{C}}}\rightarrow\mathcal{T}$ (resp. $\mathcal{T}^{\underline{\mathbf{D}}}\rightarrow\mathcal{U}$) be an unramified $\underline{\mathbf{C}}$-pre-Fermat (resp.  $\underline{\mathbf{D}}$-pre-Fermat) pregeometry which is compatible with truncations. Let $\theta:\mathcal{T}\rightarrow\mathcal{U}$ be a transformation of pregeometries, and suppose there exists a natural equivalence of functors

$$F\circ(-)^{alg}_{\underline{\mathbf{C}}}\circ G_{\theta}\Rightarrow(-)^{alg}_{\underline{\mathbf{D}}}$$

\begin{thm}\label{thm:effectiveepiembedding}
Let $\mathbf{dSpace}\subset{}^{L}\mathbf{Top}(\mathcal{U})$ be a full subcategory consisting of objects which have constructibly convergent Postnikov towers. Furthermore let $\mathbf{dAff}\subset\mathbf{dSpace}$ be a subcategory, and suppose that 
\begin{enumerate}
\item
For any $X\in\mathbf{dAff}$ and $Y\in\mathbf{dSpace}$  such that $t_{0}Y\rightarrow Y$ is an equivalence the map
$$\mathbf{Map}_{\mathbf{dSpace}}(Y,X)\rightarrow\mathbf{Map}(G_{\theta},G_{\theta}(Y))$$
is an equivalence
\item
%For any $X\in\mathbf{dAff}$ there is a full subcategory $\mathbf{F}_{X}\subset{}_{X}\mathbf{Mod}$ such that
%\begin{enumerate}
%\item
%$\mathbb{L}^{\mathcal{U}}_{X\big\slash X'}\in\mathbf{F}_{X}$ for any map $X\rightarrow X'$ in $\mathbf{dAff}$.
%\item
%for any $\mathcal{F}\in\mathbf{F}_{X}$ and each $n\in\mathbb{Z}$ the natural map $\Gamma(X,\mathcal{F})\otimes^{\mathbb{L}}_{\Gamma(X)}\mathcal{O}_{X}\rightarrow\mathal{F}$ is an equivalence.
%\item
%$\psi(X)(\mathbb{L}^{\mathcal{T}}_{G_{\theta}(X)})\in\mathbf{F}_{X}$
\item
the functor $(-)^{alg}_{\underline{\mathbf{D}}}$ is conservative.
%\end{enumerate}
\item
there is a subcategory $\mathcal{T}^{sm}\subseteq\mathrm{Alg_{T}}$ such that for any $X\in\mathbf{dAff}$ there is a closed immersion $X\rightarrow\theta(T)$ for some $T\in\mathcal{T}^{sm}$.
\item
for any $T\in\mathcal{T}^{sm}$ the map
$$\psi(\theta(T))(\mathbb{L}^{\mathcal{T}}_{T})\rightarrow\mathbb{L}^{\mathcal{U}}_{\theta(T)}$$
is an equivalence. 
\end{enumerate}
Then for any $X\in\mathbf{dAff}$ and $Y\in\mathbf{dSpace}$  the map
$$\mathbf{Map}_{\mathbf{dSpace}}(Y,X)\rightarrow\mathbf{Map}(G_{\theta}(Y),G_{\theta}(X))$$
is an equivalence
\end{thm}

\begin{proof}
It suffices to show that for any $X\in\mathbf{dAff}$ the map
$$\psi(X)(\mathbb{L}_{\Gamma^{\theta}(X)}^{\mathcal{T}})\Rightarrow\mathbb{L}_{X}^{\mathcal{U}}$$
is an equivalence. For $X=\theta(T)$ this is true by assumption. For general $X$ there is a closed immersion
$$f:X\rightarrow\theta(T)$$
It suffices to prove that the map
$$\psi(X)(\mathbb{L}_{\Gamma^{\theta}(X)\big\slash \Gamma^{\theta}(\theta(T))}^{\mathcal{T}})\Rightarrow\mathbb{L}_{X\big\slash\theta(T)}^{\mathcal{U}}$$
is an equivalence. We have
%$$\psi(X)(\mathbb{L}_{\Gamma^{\theta}(X)\big\slash T}^{\mathcal{T}})\cong F(\mathbb{L}_{\Gamma^{\theta}(X)\big\slash \Gamma^{\theta}(\theta(T)}^{\mathcal{T}})\otimes^{\mathbb{L}}_{\Gamma(X)}\mathcal{O}_{X}$$
%and 
%$$\mathbb{L}_{X\big\slash\theta(T)}^{\mathcal{U}}\cong\mathbb{L}^{\mathcal{U}}_{\Gamma(X)\big\slash\Gamma(\theta(T))}\otimes^{\mathbb{L}}_{\Gamma(X)}\mathcal{O}_{X}$$
%since $\mathbb{L}_{X\big\slash\theta(T)}^{\mathcal{U}}\in\mathbf{F}_{X}$ by assumption. 
Thus it suffices to prove that 
$$F(\mathbb{L}_{G_{\theta}(X)\big\slash T)\rightarrow\mathbb{L}^{\mathcal{U}}_{X\big\slash T}$$ is an equivalence.
Now there is a closed immersion $X\rightarrow\theta(T)$, and therefore a closed immersion $G_{\theta}(X)\rightarrow T$. Thus the cotangent complexes can be computed by forgetting to $\underline{\mathbf{C}}$ and $\underline{\mathbf{D}}$ respectively. Now the claim follows by the assumption on $F$.
\end{proof}

\textcolor{red}{removeglobalsectionshere}



\subsubsection{The Filtered Case}\label{subsec:comparefermat}
As a general class of examples let $\underline{\Lambda}$ be a partially ordered abelian group, $R$ an exhaustively $\underline{\Lambda}$-filtered ring. Set $\underline{\mathbf{C}}=\mathbf{Ch}({}_{R}\mathrm{Mod}(\overline{\mathrm{Filt}}_{\underline{\Lambda}}(\mathrm{Ab})))$, and $\underline{\mathbf{D}}=\mathbf{Ch}({}_{R^{ind}}\mathrm{Mod})$. Consider the transformation of derived algebra settings
$$F:\mathbf{Ch}({}_{R}\mathrm{Mod}(\overline{\mathrm{Filt}}_{\underline{\Lambda}}(\mathrm{Ab})))\rightarrow\mathbf{Ch}({}_{R}\mathrm{Mod})$$
induced by sending a filtered object $H:\overline{\mathrm{Filt}}_{\underline{\Lambda}}(\mathrm{Ab})$ to $\colim_{\lambda}H(\lambda)$. Let $\mathrm{T}$ be an $\underline{\Lambda}$-filtered Fermat theory, which we regard as a $\underline{\mathbf{D}}=\mathbf{Ch}({}_{R}\mathrm{Mod})$-Fermat pregeometry $\mathcal{T}^{\mathrm{T}}$. Let $\mathcal{U}$ be a ${}_{R}\mathrm{Mod}$-Fermat pre-geometry, and 
$$\theta:\mathcal{T}^{\mathrm{T}}\rightarrow\mathcal{U}$$
 a fully faithful functor. Write $\mathbb{A}^{1}$ for the image of $\mathrm{Sym}(R^{ind})$ under the functor $\mathcal{T}^{\mathbf{Ch}({}_{R}\mathrm{Mod})}\rightarrow\mathcal{U}$, and let $\mathbb{A}^{1}_{\lambda}$ denote the image of $\mathrm{Sym}(R(\lambda))$ under the composition
$$\mathcal{T}^{\mathbf{Ch}({}_{R}\mathrm{Mod}(\overline{\mathrm{Filt}}_{\underline{\Lambda}}(\mathrm{Ab})))}\rightarrow\mathcal{T}^{\mathrm{T}}\rightarrow\mathcal{U}$$
Suppose that the topology $\tau$ on $\mathcal{U}$ is such that the maps $\mathbb{A}^{1}_{\lambda}\rightarrow\mathbb{A}^{1}$ induce a cover
$$\{\mathbb{A}^{1}_{\lambda}\rightarrow\mathbb{A}^{1}\}_{\lambda\in\underline{\Lambda}}$$
Then for $\mathcal{A}\in\mathbf{Str}^{loc}_{\mathcal{U}}(\mathcal{X})$ we have 
$$\mathcal{A}_{alg}=\mathcal{A}(\mathbb{A}^{1})\cong\colim_{\lambda}\mathcal{A}(\mathbb{A}_{\lambda}^{1})$$
Thus we have a naural isomorphism
$$F(G_{\theta}(\mathcal{A})^{alg})\rightarrow\mathcal{A}^{alg}$$


The functor $F$ is exact, strongly monoidal, and preserves projectives. Thus by Lemma \ref{lem:transcotangent} we have an equivalence $F(\mathbb{L}_{\mathcal{B}\big\slash\mathcal{A}})\cong\mathbb{L}_{F(\mathcal{B})\big\slash F(\mathcal{A})}$ for any map $\mathcal{A}\rightarrow\mathcal{B}$\newline
in
 $\mathbf{Shv}(\mathcal{X},\mathbf{DAlg}^{cn}(\mathbf{Ch}({}_{R}\mathrm{Mod}(\overline{\mathrm{Filt}}_{\underline{\Lambda}}(\mathrm{Ab})))))$. Thus if for each $n\in\mathbb{N}$ and each $\underline{\lambda}=(\lambda_{1},\ldots,\lambda_{n})\in\underline{\Lambda}^{n}$ we have that the map
$$\mathbb{L}_{\mathbb{A}^{1}_{\lambda_{1}}\times\ldots\times\mathbb{A}^{1}_{\lambda_{n}}}\rightarrow\mathcal{O}_{\mathbb{A}^{1}_{\lambda_{1}}\times\ldots\times\mathbb{A}^{1}_{\lambda_{n}}}^{n}$$
is an equivalence, we can apply the discussion above to this setup.


\subsection{Strictifying and Embedding the Analytic Pre-Geometries}


Let $k$ be either $\mathbb{C}$ or a non-trivially valued non-Archimedean Banach field.

Consider the pregeometry $\mathcal{T}_{an}(k)$ defined in \cite{https://arxiv.org/pdf/1601.00859.pdf} as follows. 

\begin{enumerate}
\item
The underlying category of $\mathcal{T}_{an}(k)$ is the category of smooth $k$-analytic spaces (rigid in the case that $k$ is a non-Archimedean field).
\item
A morphism in $\mathcal{T}_{an}(k)$ is admissible precisely if it is \'{e}tale.
\item
The topology on $\mathcal{T}_{an}(k)$ is the \'{e}tale topology.
\end{enumerate}




\subsubsection{The Stein Case}
There is a fully faithful transformation of pregeometries

$$\mathcal{T}^{\mathrm{LT}^{\mathrm{EFC}_{k}}}\rightarrow\mathcal{T}_{an}(k)$$

The following is shown in \cite{https://arxiv.org/pdf/1805.08538.pdf}.

\begin{prop}[ \cite{https://arxiv.org/pdf/1805.08538.pdf}, Proposition 3.25]
Let $\mathbf{dStn}^{PYY}_{k}$ denote the category of derived $k$-analytic spaces $X$ in the sense of Porta and Yue Yu such that $t_{0}X$ is a finitely embeddable Stein space. Then the functor
$$\Gamma^{\mathrm{LT}^{\mathrm{EFC}_{k}}}:(\mathbf{dStn}^{PYY}_{k})^{op}\rightarrow\mathbf{sAlg}_{\mathrm{LT}^{\mathrm{EFC}_{k}}}$$
is fully faithful.
\end{prop}

\begin{prop}[\cite{Pridham}  Proposition 4.5]
Thee essential image of $\Gamma$ consists of those $\mathrm{EFC}_{k}$-algebras $A$ such that $\pi_{0}(A)$ is the $\mathrm{EFC}_{k}$-algebra of analytic functions on a Stein space, and $\pi_{n}(A)$ is finitely generated as a $\pi_{0}(A)$-module.
\end{prop}


\subsubsection{The Affinoid Case}

For $k$ non-Archimedean there is also an evident natural transformation of pregeometries
$$\theta:\mathcal{T}^{\mathrm{Tate}_{k}}\rightarrow\mathcal{T}_{an}(k)$$
By \cite{https://www.math.ias.edu/~lurie/papers/DAG-V.pdf} Proposition 3.2.8 the pregeometry $\mathcal{T}_{an}(k)$ is Morita equivalent to the pregeometry $\mathcal{T}_{Afnd}(k)$, which is the full subcategory of $\mathcal{T}_{an}(k)$ consisting of smooth affinoids with the Grothendieck topology and the class of admissible morphisms inherited from $\mathcal{T}_{an}(k)$.
Let $\mathbf{dAff}$ denote the category of derived affinoids.

Consider the functor
$$\Gamma:\mathrm{An}^{op}_{k}\rightarrow\mathrm{Alg}_{\mathrm{Tate}_{k}}$$
$$\Gamma(X)(\lambda)\defeq\mathrm{Hom}_{\mathrm{An}_{k}}(X,\mathcal{M}(k<\lambda>))$$

\begin{lem}
The functor $k<\gamma>\mapsto\mathrm{Hom}_{{}_{k}\mathrm{Alg}}(k<\gamma>,k<1,\ldots,1>\big\slash I)$ is a finitely presented $\mathrm{Tate}_{k}$-algebra.
\end{lem}

\begin{proof}
This is not as immediate as one might assume. Indeed, the trnasformation of functors  $\mathrm{Hom}_{{}_{k}\mathrm{Alg}}(-,k<1,\ldots,1>)\rightarrow\mathrm{Hom}_{{}_{k}\mathrm{Alg}}(-,k<1,\ldots,1>\big\slash I)$ will not in general be an epimorphism unless $I$ is radical. First, we claim that the map
$$\mathrm{Hom}_{{}_{k}\mathrm{Alg}}(-,k<1,\ldots,1>)\rightarrow \mathrm{Hom}_{{}_{k}\mathrm{Alg}}(-,k<1,\ldots,1>\big\slash(x_{1}^{m_{1}},\ldots,x_{n}^{m_{n}}))$$
is an epimorphism. First consider the case $n=1$. Let $\phi:k<\gamma>\rightarrow k<1>\big\slash(x^{m})$. This corresponds to picking an element $[f(x)]\in k<1>\big\slash(x^{m})$. We may represent $f(x)$ as $f(x)=x^{l}g(x)$ where $x$ does not divide $g(x)$. Then $[g(x)]$ is not nilpotent, so there is a $C$ such that $||[g(x)]||\le C\rho([g(x)])^{n}$. 


%Let $\phi:k<\gamma>\rightarrow k<1,\ldots,1>\big\slash(x_{1}^{m_{1}},\ldots,x_{n}^{m_{n}})$ be a map. This corresponds to selecting an element $[f(\underline{x})]\in k<1,\ldots,1>\big\slash(x_{1}^{m_{1}},\ldots,x_{n}^{m_{n}})$. We may write this as a sum $\underline{x}^{I_{1}}[f_{1}(\underline{x})]+\ldots+\underline{x}^{I_{k}}[f_{k}(\underline{x})]$ where the $f_{i}$ are not nilpotent. Note that for each $i$ there is a $C_{i}$ such that $||[f_{i}(\underline{x})]||\le C_{i}\rho$



\end{proof}

\begin{lem}
Let $X$ be affinoid and $Y$ be any analytic space. Then the natural map
$$Hom_{An_{k}}(Y,X)\rightarrow Hom_{\mathrm{Alg}_{\mathrm{Tate}_{k}}}(\Gamma(X),\Gamma(Y))$$
is an equivalence. Moreover when restricted to the category of strictly affinoid spaces $\Gamma$ determines an anti-equivalence with the category of  strictly finitely presented $\mathrm{Tate}_{k}$-algebras. \textcolor{red}{definesometerms}
\end{lem}

\begin{proof}
For the first claim we may also assume that $Y$ is also an affinoid.
Let 
$$\alpha:Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\lambda}>\big\slash I)\rightarrow Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\gamma}>\big\slash J)$$
be a natural transformation. Denote by $\pi_{I}:k<\underline{\lambda}>\rightarrow k<\underline{\lambda}>\big\slash I$ the projection. Let $\alpha_{\underline{\lambda}}$ denote the component of $\alpha$ evaluated at $k<\underline{\lambda}>$ and write $\beta=\alpha_{\underline{\lambda}}(\pi_{I}):k<\underline{\lambda}>\rightarrow k<\underline{\gamma}>\big\slash J$. Let $g\in I$ with $||g||=\delta$. Consider the two maps $f_{g},f_{0}:k<\delta>\rightarrow k<\underline{\lambda}>$ induced by sending the generating variable $x$ to $g$ and $0$ respectively. The composites $\pi_{I}\circ f_{g}=\pi_{I}\circ f_{0}$ are equal. This implies that $\alpha_{\underline{\lambda}}(\pi_{I})\circ f_{h}=\alpha_{\underline{\lambda}}(\pi_{I})\circ f_{0}$. In particular $\alpha_{\underline{\lambda}}(\pi_{I})(g)=0$, so $\alpha_{\underline{\lambda}}(\pi_{I})(g)$ descends to a map $\overline{\alpha}:k<\underline{\lambda}>\big\slash I\rightarrow k<\underline{\gamma}>\big\slash J$. Moreover $\alpha=Hom_{{}_{k}\mathrm{Alg}}(-,\overline{\alpha})$. Let $\phi,\psi:k<\underline{\lambda}>\big\slash I \rightarrow k<\underline{\gamma}>\big\slash J$ be maps such that the induced maps
$$\overline{\phi},\overline{\psi}:Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\lambda}>\big\slash I)\rightarrow Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\gamma}>\big\slash J)$$
coincide. This implies that $\phi\circ\pi_{I}=\psi\circ\pi_{I}$, which clearly implies that $\phi=\psi$.

Now let $k<\underline{\lambda}>\big\slash I$ be a strictly smooth affinoid algebra. To show that $Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\lambda}>\big\slash I)$ is finitely presented it suffices to show that $Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\lambda}>\big\slash I)\rightarrow Hom_{{}_{k}\mathrm{Alg}}(-,k<\underline{\lambda}>\big\slash I)$. Let $f:k<\gamma>\rightarrow k<\underline{\lambda}>\big\slash I$ be a map. THis is necessarily bounded and completely determined by where it sends the variable $x$ on the left-hand side. 
\end{proof}


\begin{thm}
Let $X$ and $Y$ be derived analytic spaces in the sense of \cite{PYY}, with $X$ being a derived affinoid. Then the natural map
$$\mathbf{Map}_{\mathbf{dAn}}(X,Y)\rightarrow\mathbf{Map}_{\mathbf{sAlg}_{\mathrm{Tate}_{k}}}(\Gamma(Y),\Gamma(X))$$
is an equivalence. 
\end{thm}

\begin{proof}
For $Y$ a derived analytic space denote by $\mathbf{F}_{Y}$ the category of coherent sheaves on $Y$. This category satisfies the assumptions of Theorem \ref{thm:effectiveepiembedding} by Cartan's Theorem A for affinoids
\end{proof}

\begin{thm}
The essential image of $\Gamma:\mathbf{dAn}_{k}\rightarrow\mathbf{sAlg}_{\mathrm{Tate}_{k}}$ consists of those algebras $A$ such that $\pi{0}(A)$ is the $\mathrm{Tate}_{k}$-algebra of functions on a \textcolor{red}{strict?} affinoid and $\pi_{n}(A)$ is a trivially filtered $\pi_{0}(A)$-module which is finitely generated as a $\overline{\pi_{0}(A)}$-module.
\end{thm}

\begin{proof}
Write $\pi_{0}(A)=\Gamma(X)$ with $X$ an affinoid. Let $\mathbb{O}^{A}$ denote the $\mathcal{T}_{an}(k)$-structured simplicial set defined on a smooth $k$-analytic space $U$ by
$$U\mapsto\mathbf{Map}_{\mathbf{sAlg}_{\mathrm{Tate}_{k}}}(\Gamma(U),A)$$
We claim that this does in fact define a $\mathcal{T}_{an}(k)$-structure. 
\textcolor{red}{fix:finish}
\end{proof}





%In this section we fix a pregeometry $\mathcal{U}$, and investigate to what extent subcategories of ${}^{L}\mathbf{Top}(\mathcal{U})$ may be determine by restriction to discrete sub-pregeometries $\mathcal{T}\subset\mathcal{U}$. To be precise let $\theta:\mathcal{T}\subset\mathcal{U}$ be a full subcategory such that
%\begin{enumerate}
%\item
%$\mathcal{U}$ consists of $0$-truncated objects.
%\item
%Whenever $f:X\rightarrow Y$ is an admissible monomorphism in $\mathcal{U}$ between objects in $\mathcal{T}$, then $f$ is an isomorphism. 
%\item
%For any $X\in\mathcal{U}$ and $Y\in\mathcal{T}$ the map
%$$\mathbf{Map}_{\mathcal{U}}(X,\theta(Y))\rightarrow\mathbf{Map}_{\mathbf{Str}^{loc}_{\mathcal{T}}(\mathbf{sSet})}(\Gamma^{\theta}(Y),\Gamma^{\theta}(X))$$
%is an equivalence.
%\end{enumerate}
%
%
%Let 
%
%$$({}^{L}\mathbf{Top}(\mathcal{T}),\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta,\mathbf{dSpace},\mathbf{F})$$
%be a relative pre-$(\infty,1)$-algebro-geometric tuple. 
%
%Let $\mathbf{dSpace}\subset{}^{L}\mathbf{Top}(\mathcal{U})$ be a full subcategory consisting of objects $X=(\mathcal{X},\mathcal{O}_{X})$ such that
%\begin{enumerate}
%\item
%$t_{0}(X)\in\mathcal{U}$
%\item
%For any $U\in\
%\end{enumerate}
%and let $\mathbf{dAff}\subset\mathbf{dSpace}$ denote the full subcategory consisting of objects $Y=(\mathcal{Y},\mathcal{O}_{Y})$ such that $t_{0}(Y)\in\mathcal{T}$. 
%
%
%We will generally use this result in the following situation. Assume that 
%\begin{enumerate}
%\item
%For any $X\in\mathbf{dAff}$ $\mathbb{L}_{X}$ is projective and in tor-amplitude $0$ relative to $(\mathbf{dAff},\mathbf{F})$.
%\item
%For any $X\in\mathbf{dAff}$ the map
%$$\colim t_{\le n}(X)\rightarrow X$$
%is an equivalence.
%\item
%For any $X\in\mathbf{dAff}$ there is an effective epimorphism 
%\end{enumerate}
 
% Let $\phi:\mathcal{T}\rightarrow\mathcal{U}$ be a transformation of pregeometries, let $\mathcal{X}$ be an $\infty$-topos, and let $\mathcal{O}_{X}\in\mathbf{Str}_{\mathcal{U}}^{loc}(\mathcal{X})$. There is an induced functor
% $$\phi_{*}:\mathbf{Str}_{\mathcal{U}}^{loc}(\mathcal{X})_{\big\slash \mathcal{O}_{X}}\rightarrow\mathbf{Str}_{\mathcal{T}}^{loc}(\mathcal{X})_{\big\slash \phi_{*}(\mathcal{O}_{X})}$$




%Let $(G,\phi,\deta,\epsilon)$ be a morphism of pre-$(\infty,1)$-algebro-geometric tuples from
%$$(\mathbf{Aff},\mathbf{Str},\mathcal{O},\mathrm{Spec},\eta)$$
%to $\mathbf{Aff_{C}}$, where $\mathbf{Aff}$ has a terminal object $\bullet$. 






%\subsection{Topologies}

